On Sparse Modern Hopfield Model

We introduce the sparse modern Hopfield model as a sparse extension of the modern Hopfield model. Like its dense counterpart, the sparse modern Hopfield model equips a memory-retrieval dynamics whose one-step approximation corresponds to the sparse attention mechanism. Theoretically, our key contribution is a principled derivation of a closed-form sparse Hopfield energy using the convex conjugate of the sparse entropic regularizer. Building upon this, we derive the sparse memory retrieval dynamics from the sparse energy function and show its one-step approximation is equivalent to the sparse-structured attention. Importantly, we provide a sparsity-dependent memory retrieval error bound which is provably tighter than its dense analog. The conditions for the benefits of sparsity to arise are therefore identified and discussed. In addition, we show that the sparse modern Hopfield model maintains the robust theoretical properties of its dense counterpart, including rapid fixed point convergence and exponential memory capacity. Empirically, we use both synthetic and real-world datasets to demonstrate that the sparse Hopfield model outperforms its dense counterpart in many situations.

==> 2method.tex <==
To be filled.

We simply replace softmax with $\alpha$-entmax \cite{peters2019sparse} in the attention heads, and investigate the theoretical aspects of the corresponding sparse Hopfield.
Crucially, entmax transforms are sparse for all $\alpha > 1$.


\subsection{Transformer}

The transformer is a sequence-to-sequence model that maps the input sequence to an output sequence through multi-head attention mechanisms.

Transformer consists four components:
\begin{itemize}
    \item attetion
    \item MLP
    \item residual connection
    \item layer normalization
\end{itemize}

\paragraph{Attention Mechanism.}
The index set $\{1,\cdots,I\}$ is denoted by $[I]$, where $I\in\mathbb{N}^+$. 
The spectral norm is denoted by $\norm{\cdot}_2$, which is equivalent to the $l_2$-norm when applied to a vector. The Frobenius norm is denoted by $\norm{\cdot}_{\text{F}}$. 

An attention function maps a query and a set of attended key-value pairs to an output,
where the query, keys, values, and output are all vectors.

For an input sequence $X=\{\bx_l\}_{l\in[L]}$ with the input tokens $\bx_l\in\mathbb{R}^N$, we consider the \textit{key} matrix $K\in \mathbb{K}^{L\times N_p}$ and the \textit{value} matrix $V\in \mathbb{R}^{L\times N}$ given as
\begin{align}
    K&\coloneqq\(\bk_1,\cdots,\bk_L\)^\sT=\(\bk_\theta(\bx_1),\cdots,\bk_\theta(\bx_l)\)^\sT\in \mathbb{R}^{L\times N_p},
    \\
    V&\coloneqq\(\bv_1,\cdots,\bv_L\)^\sT=\(\bv_\theta(\bx_1),\cdots,\bv_\theta(\bx_l)\)^\sT\in \mathbb{R}^{L\times N},
\end{align}
where $\bk_\theta(\cdot):\R^{N}\to \R^{N_p}$ and $\bv_\theta(\cdot):\R^{N_p}\to \R^{N}$ are learned functions with parameter $\theta\in\Theta$, mapping the $l$-th input token $\bx_l$ to its corresponding key $\bk_\theta(\bx_l)$ and value $\bv_\theta(\bx_l)$, respectively.

Formally, for any query vector $\bq\in\R^{N_p}$, the attention mechanism \cite{vaswani2017attention} computes a vector of attention scores weighted by attended value $V$
\bea
\mathsf{Attn}\(\bq, K,V\)\coloneqq V^\sT \mathsf{Norm}\[\calK\(K,\bq\)\]\in\R^N,
\eea
where $\calK\(\cdot,\cdot\):\R^{N_p}\times \R^{N_p}\to \R$ represents a kernal function, and $\mathsf{Norm}\[\cdot\]:\R^L\to \R^L$ is an element-wise normalization map.
For later convenience, we shorthand $\calK\(K,\bq\)=\(\calK\(\bk_l,\bq\)\)_{l\in[L]}\in\R^L$.



Concretely, in \cite{vaswani2017attention}, the attention mechanism is the softmax attention where 
the kernel is the
exponential kernel $\calK(\bk_l,\bq)\coloneqq \exp{\beta \bk_l^\sT \bq}$ with a fixed softmax inverse temperature $\beta>0$, and $\mathsf{Norm}\[\cdot\]$ is the softmax normalization
\bea
\mathsf{Norm}\[\calK\(K,\bq\)\]=
\mathsf{Norm}\[\(\cdots,\calK\(\bk_l,\bq\),\cdots\)_{l\in[L]}\]
=\frac{\calK\(K,\bq\)}{\sum_l \calK\(\bk_l,\bq\)}\in \R^{L},
\eea
such that
\bea
\label{eqn:attention_def}
\mathsf{Attn}\(\bq, K,V\)=V^\sT \Softmax\({\beta K^\sT \bq}\) \in\R^N.
\eea
In NLP, an input sequence $X$ is composed of word embeddings in a paragraph, while in CV, it is composed of patch embeddings in an image.

\begin{definition}[Self-Attention \cite{vaswani2017attention}]
Let $X\in \R^{N \times L}$ a data point (a sequence of length $L$) and $\calP\in \R^{N\times L}$ its positional encoding.
The self-attention mechanism computes
\begin{enumerate}
    \item the sum of sequences and positional encodings: $\Tilde{X} \coloneqq X+\calP \in \R^{N\times L}$, i.e. in practice, positional encoding  is incorporated
    additively  instead of concatenation.

    \item 
    the attention matrix $A=QK^\sT$, where
    $Q={\Tilde{X}}^\sT W_Q$, $K=\Tilde{X}^\sT W_K$ with $W_Q,W_K\in \R^{N \times N}$.
    \item
    the score/similarity matrix $\Softmax\( \beta A\)\in \R^{L\times L}$ with $\beta = 1/\sqrt{N}$.

    \item the value matrix $V=\Tilde{X}^\sT W_V$ with $W_V\in \R^{N\times N}$.
\end{enumerate}
    Lastly, it outputs the attention score
    \bea
    \mathsf{Attn}\(X,P\)=\mathsf{Attn}\(K,Q,V\)=\Softmax\({\beta QK^\sT}\)V \in\R^{N\times L}.
    \eea
\end{definition}




\subsection{Sparse Attention via $\alpha$-\sf{entmax}}



\subsubsection{Sparsemax}
\begin{claim}
The difference between softmax and sparsemax: the choice of entropic regularizer.
Therefore, the interpolations between different entropic regularizers lead to a general notion of sparsemax.
\end{claim}
The softmax transformation has a limitation in that the resulting probability distribution is always dense, with non-zero probabilities assigned to all possible outcomes, i.e.
$\Softmax_i(\bz) \neq 0$ for $i$.
This can be problematic in situations where a sparse probability distribution is desired. 
To address this issue, a threshold can be defined below which small probability values are truncated to zero, leading to a sparse distribution.


\begin{definition}[Unit Simplex]
    The $(N)$-dimensional unit simplex is defined as $\Delta^{N}\coloneqq\{\bz\in\R^N|\norm{\bz}_1,z_i\ge0\; \forall i\}$.
    Intuitively, $\Delta^N$ represents the set of vectors representing
    probability distributions over $N$ choices.
\end{definition}
\begin{definition}[Softmax]
    For any $\bz\in\R^N$ and $\beta>0$, the softmax function is given by
    \bea
    \Softmax(\bz)\coloneqq\frac{1}{\sumN \exp{\beta z_i}}\(\exp{\beta z_1},\cdots,\exp{\beta z_N}\)^\sT,
    \eea
    where each element takes the form:
    $\Softmax_i(\bz)\coloneqq\frac{\exp{\beta z_i}}{\sum_{j=1}^N\exp{\beta z_j}}$.
    Notably, $\Softmax:\R^N\to \Delta^{N-1}$ converts a vector of real values (e.g., label scores) to a probability distribution (e.g. posterior of labels).
    The $\Softmax$ has another variational form
    \bea
    \label{eqn:variational_softmax_def}
    \Softmax(\bz)\coloneqq\argmax_{\bp\in\Delta^N}\[\bp^\sT \bz-\sum_jp_j\ln p_j\].
    \eea
\end{definition}
\begin{lemma}
\label{lemma:grad_lse}
    The $\Softmax$ is the gradient of $\lse$: $\Softmax\(\beta \ba\)=\grad_{\ba} \lse\(\beta,\ba\)$.
\end{lemma}
\begin{lemma}[Lemma~A19 of \cite{ramsauer2020hopfield}]
\label{lemma:lse_properties}
    Given $\bz,\bx\in\R^N$, and $(N-1)$-dimensional unit simplex $\Delta^{N-1}\coloneqq\{\bz|\sumN z_i=1,z_j\ge0\;\forall j\}$.
    Consider a $\bz$-parametrized linear model regularized by negative entropy restricted to the simplex $\Delta^{N-1}$ with object function $\calL(\bx,\bz)\coloneqq \bz^\sT \bx
    -\frac{1}{\beta} \sumN z_i\ln z_i$,
    with $ \bz^\sT \bx\ge 0$.
    \begin{itemize}
        \item The $\lse$ is the maximum of $\calL$ on $\Delta^{N-1}$: $\lse(\beta,\bx)=\max_{\bz\in\Delta^{N-1}}\calL(\bz)$.
        \item The $\Softmax(\beta\bx)$ is the argmax of $\calL$ on $\Delta^{N-1}$: 
        $\Softmax(\beta\bx)=\argmax_{\bz\in\Delta^{N-1}} \calL(\bz)$.
    \end{itemize}
\end{lemma}

\citet{martins2016softmax} propose sparsemax, a differentiable sparse mapping from $\R^N$ to $\Delta^N$, as an alternative to softmax fucntion to compute attention scores:
\bea 
\label{eqn:sparsemax}
\Sparsemax(\bz)\coloneqq\argmin_{\bp\in\Delta^N}\norm{\bp-\bz}^2
\leftrightarrow 
\Sparsemax(\bz)=\argmax_{\bp\in\Delta^N}\[\bp^\sT\bz + 
 \half \sum_j p_j(1-p_j)\]
,
\eea 
where $\half \sum_j p_j(1-p_j)$ is known as the Gini entropy. \jhcomment{How to prove \eqref{eqn:sparsemax}?}

\red{[Key connection to sparse Hopfield: Is there any function $F(\cdot)$ such that $\grad_{\bz} F(\bz)=\Sparsemax(\bz)$?]}

The $\Sparsemax$ \eqref{eqn:sparsemax} naturally induce a projection on $\Delta^N$ resulting to a sparse predictive distribution $\bp^\star\coloneqq\Sparsemax(\bz)$ over $\bz$.
Notably, $\bp^\star$ assigns exactly zero probability to low-scoring labels.
In addition, the Jacobian properties of $\Sparsemax$ has been investigated 
\bea
\pdv{\Sparsemax(\bz)}{\bz}=\diag(\bs)-\frac{1}{\norm{\bs}}\bs^\sT\bs,
\quad
\grey{
\[\text{c.f. } \pdv{\Softmax(\bz)}{\bz}=\diag(\bp)-\bp^\sT\bp\]
}
\eea
where, for all $j\in[N]$, $s_j=1$ if $p^\star_j>0$, otherwise $s_j=0$.



Consequently, the standard negative log likelihood loss based on softmax is replaced with 
\bea
\calL_{\Sparsemax}(y,\bz)\coloneqq \norm{\be_y-\bz}^2-\norm{\bp^\star- \bz}^2,
\eea
where $\be_y\coloneqq(0,\cdots,\underbrace{1}_y,\cdots,0)$ is the indicator vector at $y$.
The gradient of $\calL_{\Sparsemax}$ is given by
\bea
\grad_{\bz} \calL_{\Sparsemax}(y,\bz)= \bp^\star -\be_y,
\eea
and hence is well-defined for training.





\subsection{Sparse Hopfield Family}


\begin{definition}[Sparse Hopfield]
\label{def_sparsemax_hopfield}
Hopfield energy:
\bea
\label{eqn:sparsemax_hopfield}
\red{\calH_{\Sparsemax}\coloneqq???}
\eea
Retrieval dynamics:
\bea
\bxi^{\textbf{new}}= \bm{\Xi}^\sT \Sparsemax\(\bm{\Xi}^\sT \bxi\).
\eea
Note that, 
\bea
\grad \calH_{\Sparsemax} = \bxi^{\textbf{new}}= \bm{\Xi}^\sT \Sparsemax\(\bm{\Xi}^\sT \bxi\).
\eea
\end{definition}  





\begin{definition}[$\alpha$-{\sf{entmax}} Hopfield Family]
\label{def_entmax+hopfield}
Hopfield energy:
\bea
\label{eqn:sparsemax_hopfield}
\red{\calH_{\text{$\alpha$-{\sf{entmax}}}}\coloneqq???}
\eea
Retrieval dynamics:
\bea
\bxi^{\textbf{new}}= \bm{\Xi}^\sT {\text{$\alpha$-{\sf{entmax}}}}\(\bm{\Xi}^\sT \bxi\).
\eea
Note that, 
\bea
\grad \calH_{\text{$\alpha$-{\sf{entmax}}}} = \bxi^{\textbf{new}}= \bm{\Xi}^\sT {\text{$\alpha$-{\sf{entmax}}}}\(\bm{\Xi}^\sT \bxi\).
\eea
\end{definition}  

\begin{problem}
\label{prob_main}
   To obtain Hopfield models in Definition~\ref{def_sparsemax_hopfield} \& \ref{def_entmax+hopfield}, we consider the following optimization problem
\bea
\grad_\bx \calH(\bx)=\argmax_{\bp\in\Delta^N}\[\bp^\sT\bx -\Psi(\bp)\],
\eea
and solve for $\calH(\bx)$.  
Note that, the entropic regularizer $\Psi$ controls the sparsity. 
\end{problem}


\begin{itemize}
    \item For $\Sparsemax$, $\Psi(\bp)=-\half \sum_j p_j(1-p_j)$.

    \item
    For $\text{$\alpha$-{\sf{entmax}}}$, 
    \bea
    \Psi_\alpha(\bp)=\begin{cases}
    \frac{1}{\alpha(1-\alpha)}\sum_j\(p_j-p_j^\alpha\),\quad&\alpha\neq 1,\\
    -\sum_j p_j\ln p_j,\quad&\alpha=1.
    \end{cases}
    \eea
\end{itemize}

\clearpage

\subsubsection*{$\Softmax$ in Variational Form}




\begin{lemma}[$\Softmax$ in Variational Form]
Consider the regularized argmax function
\bea
\label{eqn:variational_softmax}
M(\bz)\coloneqq\argmax_{\bp\in\Delta^N}\[\bp^\sT\bz-\Psi(\bp)\],
\eea
where $\Psi:\R^N\to \R\cup \{+\infty\}$ is the \textit{$\lambda^{-1}$-convex} negative entropic regularizer.
If we pick
\bea
\Psi(\bp)\coloneqq \lambda^{-1} \sum_j p_j\ln p_j\quad \text{if $\bp\in \Delta^N$, otherwise $+\infty$},
\eea
then, by invoking KKT conditions, the unique maximizer of \eqref{eqn:variational_softmax} is $\Softmax$ evaluated at $\bz\in\R^N$:
\bea
\Softmax(\bz)=\bp^\star=\argmax_{\bp\in\Delta^N}\[\bp^\sT\bz-\lambda^{-1} \sum_j p_j\ln p_j \].
\eea
\end{lemma}

\begin{corollary}[$\lse$ as the Convex Conjugate of $\Psi$] 
By the definition of the Legendre-Fenchel transform, $\max_{\bp\in\Delta^N}\[\bp^\sT\bz-\lambda^{-1} \sum_j p_j\ln p_j \]$ is given by the convex conjugate of the negative entropy $\Psi(\bp)$:
\bea
\max_{\bp\in\Delta^N}\[\bp^\sT\bz-\lambda^{-1} \sum_j p_j\ln p_j \]
=\lse(\lambda,\bz)
=\lambda^{-1} \ln \[\sum_j \exp{\lambda z_j}\].
\eea
\end{corollary}








==> 2theory.tex <==

\subsection{Sparse Modern Hopfield Model and Sparse Retrieval Dynamics}


We propose the sparse Hopfield energy of the form
\bea
\label{eqn:H_sparsemax}
\boxed{
\calH_{\Sparsemax}(\bx)=-\Psi^\star\(\bm{\Xi}^\sT \bx\) +\half \Braket{\bx,\bx}
},
\eea
with
\bea
\Psi^\star(\bz)
    =
    \half \norm{\bz}^2+\half-\half\norm{\Sparsemax(\bz)-\bz}^2,
\eea
and the corresponding sparse retrieval dynamics of the form
\bea
\bx_{\text{new}}=\calT(\bx)=\grad \Psi^\star\(\bm{\Xi}^\sT \bx\) 
=\underbrace{\bm{\Xi}}_{\in \R^{d\times M}}\underbrace{\Sparsemax\(\bm{\Xi}^\sT \bx\)}_{\in \R^{M}}.
\eea

\begin{definition}[Sparsemax in Variational Form \cite{martins2016softmax}]
Let $\bz,\bp\in\R^M$, and $\Delta^{M}\coloneqq\{\bp\in\R^M_+ \mid \sum_\mu^M p_\mu=1\}$ be the $(M-1)$-dimensional unit simplex.
\begin{align}
\Sparsemax(\bz)&\coloneqq\argmin_{\bp\in\Delta^M}\norm{\bp-\bz}^2,\\
&=
\argmax_{\bp\in\Delta^M}\[\bp^\sT\bz -\Psi(\bp)\],
\end{align}
where $\Psi(\bp)\coloneqq -\half \sum_\nu^M p_\nu(1-p_\nu)$ is the Gini entropy.
\end{definition}
\begin{remark}
To see the equivalence of above two optimization problems, we observe
\begin{align}
    \argmax_{\bp\in\Delta^d} \[\Braket{\bp,\bz} -\Psi(\bp)\]
    &=
    \argmax_{\bp\in\Delta^d} \[\Braket{\bp,\bz} -\half\norm{\bp}^2\]\nonumber\\
    \label{eqn:sparse_equ2}
    &=\argmin_{\bp\in\Delta^d} \[-\half\(\norm{\bp}^2 +\norm{\bz}^2-2\Braket{\bp,\bz} \)\]\\
    &=\argmin_{\bp\in\Delta^d}\[\half\norm{\bp-\bz}^2\]\nonumber,
\end{align}
where the last line is obtained by inserting $\norm{\bz}^2$ as a constant in \eqref{eqn:sparse_equ2}.
\end{remark}

\begin{lemma}[Proposition~1 of \cite{martins2016softmax}]
Let $\bz\in\R^M$.
Denote $[a]_+\coloneqq \Max\{0,a\}$, $z_{(\nu)}$ the $\nu$'th element in a sorted descending $z$-sequence $\bz_{\text{sorted}}\coloneqq z_{(1)}\ge z_{(2)}\ge\ldots\ge z_{(M)}$, and 
\bea
\kappa(\bz)\coloneqq\Max\bigg\{k\in [M]\;\bigg\vert \; 1+kz_{(k)}>\sum_{\nu\le k}z_{(\nu)}\bigg\}.
\eea
Above optimization problem(s) has closed-form solution 
\bea
\label{eqn:sparsemax_exact}
\[\Sparsemax(\bz)\]_{\mu}=\[z_\mu-\tau(\bz)\]_+,
\eea
where $\tau:\R^M \to \R$ is the threshold function 
\bea\tau(\bz)=\frac{\(\sum_{\nu\le \kappa(\bz)}z_{(\nu)}\)-1}{\kappa(\bz)},
\eea  
satisfying $\sumM \[z_\mu-\tau(\bz)\]_+=1$ for all $\bz$.
Notably, $\kappa(\bz)=\abs{S(\bz)}$ where $S(\bz)=\{\mu\in[M]\;|\;\Sparsemax_\mu(\bz)>0\}$ is the support set of $\Sparsemax$.
\end{lemma}
\begin{remark}
    $\mu\in S(\bz)\Longleftrightarrow z_\mu>\tau(\bz)$.
\end{remark}
\begin{algorithm}
\caption{Sparsemax \cite{martins2016softmax}}
\begin{algorithmic}[1]
\Function{Sparsemax}{$\bz$}
    \State \textbf{Input:} $\bz\in \R^M$
    \State $\bz_\text{sorted} \gets \text{SortDescending}(\bz)$
    \State $\textbf{cumsum} \gets \text{CumulativeSum}(\bz_\text{sorted})$
    \State $\kappa(\bz) \gets \text{argmax}_k \bigl\{ k : \bz_\text{sorted}(k) + \[1 - \textbf{cumsum}(k)\]/k > 0 \bigr\}$
    \State $\tau(\bz) \gets \[1 - \textbf{cumsum}\(\kappa(\bz)\)\]/\kappa(\bz)$
    \For{$\mu \gets 1 \text{ to } M$}
        \State $\text{Sparsemax}(\bz)_\mu \ge  \max\[\bz_\mu - \tau(\bz), 0\]$
    \EndFor
    \State \Return $\text{Sparsemax}(\bz)$
\EndFunction
\end{algorithmic}
\end{algorithm}    

\begin{theorem}[Convex Conjugate of Negative Gini Entropy]
\label{thm:main_result}
Let $F(\bp)=\Braket{\bp,\bz} -\Psi(\bp)$.
Consider $\Psi$ being the negative Gini entropy, $\Psi(\bp)=-\half\sum_i p_i(1-p_i)=\half \norm{\bp}^2 -\half$, such that
 \bea
F(\bp,\bz)=\Braket{\bp,\bz} -\half\norm{\bp}^2+\half.
 \eea
We have the convex conjugate of $\Psi(\bp)$:
\begin{align}\label{eqn:PsiStar_sparse_hopfield}
    \Psi^\star(\bz)
    =
    \half \norm{\bz}^2+\half-\half\norm{\bp^\star-\bz}^2,
\end{align}
where $\bp^\star=\Sparsemax(\bz)$ is given by \eqref{eqn:sparsemax_exact}.
\end{theorem}
\begin{proof}[Proof of Theorem~\ref{thm:main_result}]
\begin{align}
    \Max_{\bp\in\Delta^d}\[\Braket{\bp,\bz} -\half\norm{\bp}^2+\half\]
    &=
    \Max_{\bp\in\Delta^d}\[\half\norm{\bz}^2+\Braket{\bp,\bz} -\half\norm{\bp}^2-\half\norm{\bz}^2+\half\]\\
    &=
    \Max_{\bp\in\Delta^d}\[\half\norm{\bz}^2+\half
    -\half\norm{\bp-\bz}^2
    \]\\
    &= 
    \half\norm{\bz}^2+\half
    -\Min_{\bp\in\Delta^d}\[\half\norm{\bp-\bz}^2
    \]\\
    &=
    \half\norm{\bz}^2+\half
    -\half\norm{\bp^\star-\bz}^2=\Psi^\star(\bz),
\end{align}
with $\bp^\star$ given by \eqref{eqn:sparsemax_exact}.
\end{proof}
\begin{corollary}
\label{coro:gamma_convex}
\red{
    $\Psi^\star$ is convex.
    And for $\Phi(\bz)\coloneqq -\gamma\half\sum_i p_i(1-p_i)$ ($\gamma$-strongly convex w.r.t. $\norm{\cdot}$), $\Psi^\star$ is $1/\gamma$-smooth w.r.t. dual norm $\norm{\cdot}_\star$.
    }
\end{corollary}
\begin{corollary}
\label{coro:grad_Psi}
The gradient of $\Psi^\star(\bz)$ gives the $\Sparsemax$ (as the argmax of $F$):
\bea
\grad \Psi^\star(\bz) = \argmax_{\bp\in\Delta^d}F
=\Sparsemax(\bz).
\eea
\end{corollary}
\begin{proof}
\cref{coro:gamma_convex} and \cref{coro:grad_Psi} are direct consequences of convex conjugation.
\end{proof}











\clearpage
\subsection{Memory Capacity}

\begin{mdframed}
\jhcomment{We put the main result of \cite{ramsauer2020hopfield} here for comparison.
Recall they use $M\coloneqq \Max_{\mu\in[N]}\norm{\bxi^\mu}$, and $\bxi,\bx\in d$.
}
\begin{lemma}[Random Pattern Storage, Theorem~3 of \cite{ramsauer2020hopfield}]
Given a failure probability $0<\delta\le 1$, and randomly chosen patterns with fixed norm $M\coloneqq K\sqrt{d-1}$.
Then, with probability $1-\delta$, the number of random patterns that can be stored is 
\bea
N\ge \sqrt{\delta}C^{\nicefrac{d-1}{4}},
\eea
where $c\coloneqq b/W_0\(\exp{a+\ln b}\)$ with $a\coloneqq\[2+\ln\(2\beta K^2\delta(d-1)\)\]/(d-1)$,  $b\coloneqq 2 \beta K^2/5$, and $W_0(\cdot)$ is the upper branch of the Lamber W function ensuring $c\ge \(2/\sqrt{\delta}\)^{4/(d-1)}$.
\end{lemma}
\begin{proof}[Proof Sketch from \cite{ramsauer2020hopfield}]\hfill
\begin{enumerate}
\item
Employ the technique in Lemma~A5 from \cite{ramsauer2020hopfield} to derive a lower bound for $\Delta_i$.
\item
Define the angle between two patterns $\bxi^\mu$ and $\bxi^\nu$ as $\alpha_{\mu \nu}$, and consider the smallest angle, $\alpha_{min}$. Replace $\Delta_i$ with $\Delta_{min}$.
\item
Utilizing the condition that a stored pattern lies on the sphere, substitute the lower bound for $\Delta_{\min}$ with the radius $M$ and $\cos(\alpha_{\min})$.
\item
Introduce the stored-failure probability $0 \leq p \leq 1$. With probability $1-p$, the pattern is stored successfully, and the lower bound on $\Delta_{\min}$ holds. Formulate a probability inequality based on this condition.
\item
Apply Lemmas A13, A14, and A15 from \cite{ramsauer2020hopfield} to restructure the inequality.
\item
Solve the Lambert $W$ function for $c$. As the solution provides a lower bound on $c$, it can be substituted to demonstrate the results of exponential capacity.
\end{enumerate}
\end{proof}
\end{mdframed}

\begin{lemma}[Lower Bound of Sparsemax]
\label{lemma:sparsemax_lower_bound}
\bea
\[\Sparsemax\(\beta \bm{\Xi}^\sT \bx\)\]_{\mu}=
\begin{cases}
a,\quad & \text{for }i\in S\(\beta \bm{\Xi}^\sT \bx\)\\
0,\quad & \text{for }i\notin S\(\beta \bm{\Xi}^\sT \bx\)
\end{cases}
\eea
$m\coloneqq\Max_{\mu\in [M]}\norm{\bxi^\mu}$, and for the ease of presentation $\kappa\coloneqq\kappa(\cdot)$.
We have
\bea
\[ \Sparsemax \(\beta \bm{\Xi}^\sT \bx\) \]_{\mu} \ge 
\red{\cdots} \ge 1- \red{\epsilon},
\eea
where $\red{\epsilon=1- \frac{1}{\kappa}\exp{\ln{\(\kappa-\[\beta \bm{\Xi}^\sT \bx \]_{\kappa}\)}}}$.
\end{lemma}
\begin{proof}[Proof of \cref{lemma:sparsemax_lower_bound}]
For the \textit{non-zero} $\Sparsemax$ component $i\in S\(\beta \bm{\Xi}^\sT \bx\)$,
\bea
[ \Sparsemax \(\beta \bm{\Xi}^\sT \bx\) ]_i =\[\beta \bm{\Xi}^\sT \bx \]_{\mu}+\frac{1-\sum_{\nu \leq \kappa} \[\beta \bm{\Xi}^\sT \bx\]_{(\nu)}}{\kappa},
\eea
and $1\ge \[\Sparsemax\(\beta \bm{\Xi}^\sT \bx\)\]_{\mu} >0$.

Since \red{$ \kappa \cdot \Max_{\nu}\[\beta \bm{\Xi}^\sT \bx \]_{ ( \nu ) } \ge  \sum_{\nu \leq \kappa} \[\beta \bm{\Xi}^\sT \bx\]_{(\nu)} $}, we have
\begin{align}
\[ \Sparsemax \(\beta \bm{\Xi}^\sT \bx\) \]_{\mu} 
&> 
\[\beta \bm{\Xi}^\sT \bx \]_{\mu}+ \frac{ 1-\kappa \Max_{\nu}\[\beta \bm{\Xi}^\sT \bx\]_{\nu}}{\kappa}\\
&\geq 
\[\beta \bm{\Xi}^\sT \bx \]_{\mu}-\Max_{\nu}\[\beta \bm{\Xi}^\sT \bx\]_{\nu} +\frac{ 1}{\kappa}\\
& = 
\beta \Tilde{\Delta}_\mu+ \frac{1}{\kappa}.
\end{align}
\end{proof}
\begin{lemma}[Lower Bound: $\Sparsemax$ v.s. $\Softmax$]
\label{lemma:sparsemax_vs_softmax}
For a given $\bz\in\R^M$, it holds
\bea
\red{
\min_{\mu\in S(\bz)}\[\Sparsemax(\bz)\]_{\mu} \ge \min_{\nu}\[\Softmax(\bz)\]_{\nu}.
}
\eea
Or
\bea
\boxed{
\[\Sparsemax(\bz)\]_\kappa\ge \[\Softmax(\bz)\]_\kappa
}
\eea
\end{lemma}
\begin{proof}[Proof of \cref{lemma:sparsemax_vs_softmax}]
Let z be a sorted descending sequence $\bz_{\text{sorted}}\coloneqq z_{(1)}\ge z_{(2)}\ge\ldots\ge z_{(M)}$. Since only first $\kappa$ terms in this sequence are non-zero value, $\min_{\mu}[\Sparsemax(z)]_\mu=[\Sparsemax(z)]_\kappa$. For $\Softmax$ sequence, since the $\Softmax$ value monotonically with respect to decreasing $z$, the minimum happens while $\mu=(M)$. Therefore, here we need to compare are $[\Sparsemax(z)]_\kappa$ and $[\Softmax(z)]_{(M)}$.
First we rewrite the $\Softmax$ function as inverse form:
\begin{align}
\frac{1}{[\Softmax(z)]_{(M)}}
&=
\frac{\sum^{N}_{\mu=1}\exp(z_{(\mu)})}{\exp(z_{(M)})}\\
&= \sum^{N}_{\mu=1} \exp(z_{(\mu)}-z_{(M)}).
\end{align}
and for $\mu \geq \kappa$, $z_{(\mu)}-z_{(M)} \geq z_\kappa-z_{(M)}$, we have
\begin{align}
\sum^{N}_{\mu=1} \exp(z_{(\mu)}-z_{(M)}) 
&=
\sum^{\kappa}_{\mu=1} \exp(z_{(\mu)}-z_{(M)})+\sum^{M}_{\mu=\kappa+1} \exp(z_{(\mu)}-z_{(M)})\\
&\geq
\kappa \exp(z_\kappa-z_{(M)}),
\end{align}
which means there are $\kappa$ components satisfy this condition. Since $\tau(z) \ge z_{(M)}$, we have
\bea
\kappa \exp(z_\kappa-z_{(M)})
\ge
\kappa \exp(z_\kappa-\tau(z)).
\eea
The inverse $\Sparsemax$ function can be expressed as
\bea
\frac{1}{[\Sparsemax(z)]_\kappa}=\frac{1}{z_\kappa-\tau(z)}.
\eea
Assuming $[\Sparsemax]_\kappa \ge [\Softmax]_{(M)}$ is true, we use mathematical induction to prove that the inequality
\bea
\kappa \exp([\Sparsemax(z)]_\kappa)
\ge
\frac{1}{[\Sparsemax(z)]_\kappa}
\eea
holds for all $\kappa$.
Let $\kappa=1$. The inequality
\bea
\exp{[\Sparsemax(z)]_\kappa} \ge \frac{1}{[\Sparsemax(z)]_\kappa}
\eea
holds, since $[\Sparsemax]_\kappa$ must be 1 to fulfill the constraint:
\bea
\sum_\mu^{\kappa} [\Sparsemax(z)]_{(\mu)}=1.
\eea
Assume this inequality is true for $\kappa=t$:
\bea
t \exp{[\Sparsemax(z)]_{(t)}}
\ge
\frac{1}{[\Sparsemax(z)]_{(t)}},
\eea
where $z_t-\tau(z)$ must less then or equal to $\frac{1}{t}$.
Next, we want to prove that the inequality
\bea
(t+1) \exp{z_{(t+1)}-\tau(z)}
\ge
\frac{1}{z_{(t+1)}-\tau(z)}
\eea
is true. By inductive hypothesis, it follows that
\bea
(t+1) \exp{z_{(t+1)}-\tau(z)}
\geq
t \exp{z_{(t)}-\tau(z)}
\geq
\frac{1}{z_{(t)}-\tau(z)}
\eea
\end{proof}

\begin{lemma}[Upper Bound of 1-Step Retrieval Error]
\label{lemma:retrieval_error_bound}
Given the stored (key) patterns matrix $\bm{\Xi}=\(\bxi^1,\cdots,\bxi^M\)\in \R^{d\times M}$ with the largest norm $m\coloneqq \max_\mu\norm{\bxi^\mu}$, and denote the (query) configurations of Hopfiled model by $\bx\in\R^d$.
Regarding the results of 
\bea
\norm{\calT\(\bx\)-\bxi^\mu}
\le \[1+\abs{\[\beta \bm{\Xi}^\sT \bx \]_{\kappa}}\]m.
\eea
\end{lemma}
\begin{proof}[Proof of \cref{lemma:retrieval_error_bound}]
Let $\calT_{\text{Dense}}$ be the retrieval dynamics of the dense modern Hopfield model \cite{ramsauer2020hopfield},
and $\epsilon_{\Sparsemax}\coloneqq \norm{\calT(\bx)-\bxi^\mu}$ and $\epsilon_{\text{Dense}}\coloneqq\norm{\calT_{\text{Dense}}(\bx)-\bxi^\mu}$ be the retrieval error of sparse and dense Hopfield model, respectively.

It holds
\begin{align}
\norm{\calT(\bx)-\bxi^\mu}-\norm{\calT_{\text{Dense}}(\bx)-\bxi^\mu}
=&\norm{\sum_{\nu=1}^{\kappa} \bxi^\nu \[\Sparsemax\(\beta \bm{\Xi}^\sT \bx\) \]_\nu-\bxi^\mu}\nonumber\\
&\quad-\norm{\sum_{\nu=1}^{\kappa} \bxi^\nu \[\Softmax\(\beta \bm{\Xi}^\sT \bx\) \]_\nu-\bxi^\mu}\\
\leq&
\norm{\sum^{\kappa}_{\nu=1}\[\Sparsemax(\beta\Xi^\sT \bx)\]\bxi^\nu }\nonumber\\
&\quad-
\norm{\sum^{\kappa}_{\nu=1} \[\Softmax\(\beta \bm{\Xi}^\sT \bx\)\] \bxi^\nu}\\
\leq& 0,
\end{align}
which gives
\bea
\epsilon_{\Sparsemax}=\norm{\calT(\bx)-\bxi^\mu} 
&\leq& 
\norm{\calT_{\text{Dense}}(\bx)-\bxi^\mu}=\epsilon_{\text{Dense}},
\eea
where $R_{\Sparsemax}$ is the retrieval error of $\Sparsemax$ and $R_{\Softmax}$ is that of $\Softmax$.

\grey{
\begin{align}
\norm{\calT\(\bx\)-\bxi^\mu}&=
\norm{\bm{\Xi}\Sparsemax\(\bm{\Xi}^\sT \bx\)-\bxi^\mu}
=
\norm{\sum_{\nu=1}^{\kappa} \bxi^\nu \[\Sparsemax\(\beta \bm{\Xi}^\sT \bx\) \]_\nu-\bxi^\mu}\nonumber\\
&\leq \norm{\bxi^\mu}+\norm{\sum^{\kappa}_{\nu=1} \[ \Sparsemax(\beta \bm{\Xi}^T x)\]_\nu \bxi^\nu}\\
&\leq 
m+\kappa\abs{\frac{\[\beta \bm{\Xi}^\sT \bx \]_{\kappa}}{\kappa}}m\\
&= 
\(1+\abs{\[\beta \bm{\Xi}^\sT \bx \]_{\kappa}}\)m.
\end{align}
}
\end{proof}

\begin{definition}[Separation of Patterns]
\label{def:separation_of_patterns}
The separation of a memory pattern $\bxi^\mu$ from all other memory patterns $\bm{\Xi}$ is defined as its minimal inner product difference to any other patterns:
\bea
\Delta_\mu\coloneqq
\Min_{\nu,\nu\neq \mu}\[\Braket{\bxi^\mu,\bxi^\mu}-\Braket{\bxi^\mu,\bxi^\nu}\]=\Braket{\bxi^\mu,\bxi^\mu}-\Max_{\nu,\nu\neq \mu }\[\Braket{\bxi^\mu,\bxi^\nu}\].
\eea
Similarly, the separation of a configuration $\bx$ from all memory patterns $\bm{\Xi}$ is given by
\bea
\Tilde{\Delta}_\mu\coloneqq
\Min_{\nu,\nu\neq \mu}\[\Braket{\bx,\bxi^\mu}-\Braket{\bx,\bxi^\nu}\].
\eea    
\end{definition}

\begin{theorem}[Well-Separation Condition]
\label{thm:well_separation}
Given the sphere
$
 S_\mu\coloneqq \big\{\bx \; \big\vert\; \norm{\bx-\bxi^\mu}\le R \le R_{\text{Dense}}\big\},
$
where $R$ is the radius of $ S_\mu$ for all $\mu$ and $R_{\text{Dense}}\coloneqq \nicefrac{1}{(\beta mM)}$ is the radius in \cite{ramsauer2020hopfield}.
The retrieved update $\calT\(\bx\)$ sits inside $ S_\mu$ if
\begin{enumerate}
    \item The starting point is inside $ S_\mu$:
    $
    \bx\in S_\mu.
    $
    \item 
    $\Delta_\mu$ satisfies the inequality:
    \bea 
    \Delta_\mu \ge 
    \frac{1}{\beta}\ln(\frac{2(M-1)m}{R})+2mR.
    \eea
\end{enumerate}
We say the sphere $S_\mu$ is well-separated from each other.
\end{theorem}

\begin{proof}[Proof of \cref{thm:well_separation}]

{\color{firebrick}
Recall \cref{thm:well_separation},
\begin{align}
\norm{\calT\(\bx\)-\bxi^\mu}
&\le  
\norm{\calT_{\text{Dense}}(\bx)-\bxi^\mu}\\
&=
\norm{\bxi^\mu-\sum^M_{\nu=1} [\Softmax(\beta \Xi^\sT \bx)]_\nu \bxi^\nu}\\
&=
\norm{(1-[\Softmax(\beta \Xi^\sT \bx)])\bxi^\mu-\sum^M_{\nu=1, \nu \neq \mu}[\Softmax(\beta \Xi^\sT \bx)]\bxi^\nu}\\
&\leq
\epsilon \norm{\bxi^\mu}+\frac{\epsilon}{M-1}\sum^M_{\nu=1, \nu \neq \mu} \norm{\bxi^\nu}\\
&\leq
2\epsilon M,
\end{align}
where $\epsilon=(N-1)\exp{-\beta \Delta_\mu}$.
}

Next we want to find the bound of $\Delta$ such that $\calT$ is a mapping from $S_\mu$ into $ S_\mu$.
For $\mu\in [M]$, by Cauchy-Schwartz inequality
\bea
\abs{\Braket{\bxi^\mu,\bxi^\mu}-\Braket{\bx,\bxi^\mu}}
\leq
\norm{\bxi^\mu-\bx} \cdot \norm{\bxi^\mu}
\leq
\norm{\bxi^\mu-\bx}m
\eea

Therefore,
\begin{align}
\Tilde{\Delta}_\mu 
&=
\Min_{\nu,\nu\neq \mu}
\[
\Braket{\bx,\bxi^\mu}-\Braket{\bx,\bxi^\nu}
+
\(\Braket{\bxi^\mu,\bxi^\mu}-\Braket{\bxi^\mu,\bxi^\nu}\)
-
\(\Braket{\bxi^\mu,\bxi^\mu}-\Braket{\bxi^\mu,\bxi^\nu}\)
\]
\\
&
\geq \Min_{\nu,\nu\neq \mu}
\[
\Braket{\bxi^\mu,\bxi^\mu}-\Braket{\bxi^\mu,\bxi^\nu}
+
\(\Braket{\bxi^\mu,\bxi^\nu}-
\Braket{\bx,\bxi^\nu}\)
-
\(\Braket{\bxi^\mu,\bxi^\mu}-
\Braket{\bx,\bxi^\mu}\)
\]
\annot{By Cauchy-Schwarz}
\\
&=
\Delta_\mu - 2 \norm{\bxi^\mu-\bx}m=\Delta_\mu-2mR,
\annot{By $\bx\in  S_\mu$}
\end{align}
where $R$ is radius of the sphere $S_{\mu}$.
From the bound on $\norm{\calT_{\text{Dense}}(\bx)-\bxi^\mu}$, we have
\bea
\norm{\calT(\bx)-\bxi^\mu}
&\leq&
\norm{\calT_{\text{Dense}}(\bx)-\bxi^\mu} 
\leq 
2 \Tilde{\epsilon} m\\
&=&
2(N-1)\exp{-\beta \Tilde{\Delta}_\mu}m\\
&\leq&
2(M-1) \exp{-\beta\(\Delta_\mu-2mR\)}m.
\eea
Since we assume that $\calT$ is a mapping from $S_\mu$ into $S_\mu$, we obtain the inequality to solve the lower bound on $\Delta_\mu$ and appropriate $R$:
\bea
2(M-1) \exp(-\beta(\Delta_\mu-2mR))m
\leq
R.
\eea
After some algebraic manipulation, this inequality can be expressed as
\bea
\Delta_\mu
\geq
\frac{1}{\beta}\ln(\frac{2(M-1)m}{R})+2mR.
\eea
Therefore, while $\Delta_\mu$ satisfies this inequality, $\calT$ is a mapping from $S_\mu$ into itself.
\end{proof}
\begin{remark}
The well-separated condition \cref{thm:well_separation} is the necessary condition for the pattern $\bxi_\mu$ according to \cref{def:stored_and_retrieved}.
\end{remark}



\begin{lemma}
\label{lemma:contraction}
The retrieval dynamics $\calT$ is a contraction mapping in $ S_\mu$ under the condition
\bea
\beta m^2M \(1-\frac{1}{\kappa}\) \leq 1
\eea
\end{lemma}
\begin{proof}[Proof of \cref{lemma:contraction}]
Let $J\coloneqq \grad_\bx \calT(\bx)$ and $\calJ_{\Sparsemax}\coloneqq \grad_{\bz} \Sparsemax(\bz)$ be the Jacobians of the retrieval dynamics \eqref{def:sparse_retrieval_dyn} and $\Sparsemax$, respectively.

Given the interpolation from $\bx$ to $\bxi^\mu$ as $\Tilde{\bx}\coloneqq \bx + (1-\lambda)\bxi^\mu$ for $\lambda\in[0,1]$, the mean value theorem yields
\bea
\calT(\bx)=\calT(\bxi^\mu)+\calJ^\mu(\bx-\bxi^\mu),
\eea
where $\calJ^\mu\coloneqq\int^1_0 \calJ(\lambda \bx+(1-\lambda)\bxi^\mu)\,\dd\lambda$.
To show $\calT$ is a contraction map in $ S_\mu$, it is sufficient to show that $ \norm{\calJ^\mu}_2<1$, resulting in
\bea
\norm{\calT(\bx)-\calT(\bxi^\mu)} \leq \norm{\calJ^\mu}_2 \norm{\bx-\bxi^\mu} \le \norm{\bx-\bxi^\mu} \le R,
\eea
or equivalently $\calT(\bx)\in S_\mu$ for all $\bx\in S_\mu$.



By \cref{lemma:sparsemax_Jacobian}, we have the maximum absolute column sum norm of Jacobian of the $\Sparsemax$ function as
\bea
\norm{\calJ_{\Sparsemax}}_1 = \beta \(1-\frac{1}{\kappa}\)
\leq
2m
\eea
and the maximum absolute row sum norm is given by
\bea
\norm{\calJ_{\Sparsemax}}_\infty = \beta \(1-\frac{1}{\kappa}\).
\eea
By Hölder's inequality, we have
\bea
\norm{\calJ_{\Sparsemax}}_2 \leq \sqrt{\norm{\calJ_{\Sparsemax}}_1\norm{\calJ_{\Sparsemax}}_\infty}=\beta \(1-\frac{1}{\kappa}\).
\eea
By chain rule, we have $\calJ=\beta\bm{\Xi}\calJ_{\Sparsemax}\bm{\Xi}^\sT$, and hence the inequality 
\bea
\norm{\calJ}_2 \leq \beta \norm{\bm{\Xi}}_2^2 \norm{\calJ_{\Sparsemax}}_2 \leq \beta \norm{\bm{\Xi}}^2_2 \(1-\frac{1}{\kappa}\),
\eea
holds.
Moreover, the spectral norm $\norm{\cdot}_2$ is bounded by Frobenius norm $\norm{\cdot}_F$:
\bea
\norm{\bm{\Xi}}_2 \le \norm{\bm{\Xi}}_F = \sqrt{\sum_\mu\norm{\bm{\xi}^\mu}^2} \leq m\sqrt{M},
\eea
which leads to the bound on $\norm{\calJ}_2$:
\bea
\norm{\calJ}_2 \leq \beta m^2 M\(1-\frac{1}{\kappa}\).
\eea
Since $\calJ^\mu$ interpolates $\calJ$ over $\lambda\in[0,1]$, the bound on $\norm{\calJ}$ also holds for $\norm{\calJ^\mu}$
\bea
\norm{\calJ^\mu}_2 \leq \beta m^2M \(1-\frac{1}{\kappa}\).
\eea
Therefore, $\calT$ is a contraction mapping if
\bea
\beta m^2M \(1-\frac{1}{\kappa}\) \leq 1,
\eea
holds.

\end{proof}

\begin{corollary}
\label{corollary:Delta_min}
Let $\Delta_{\min}=\Min_{\mu\in[M]}\Delta_\mu$.
We have
\bea
\Delta_{\min}\ge 
\frac{1}{\beta}\ln(\frac{2(N-1)M}{R})+2MR.
\eea
\end{corollary}

\begin{assumption}[Memory Patterns on a Sphere]
\label{assumption:patterns_on_sphere}
Following \cite{demircigil2017model}, we assume all memory patterns being on a sphere of radius $m$: $\norm{\bxi^\mu}=m$ for all $\mu$.
\end{assumption}
\begin{remark}
This assumption is for the ideal case, i.e. the situation of maximal memory capacity. 
\end{remark}
\begin{lemma}
\label{lemma:theta_min}
Let $\theta_{\mu\nu}$ be the angle between two patterns $\bxi^\mu$ and $\bxi^\nu$.
Following \cref{assumption:patterns_on_sphere}, we denote
\bea
\Delta_{\min}=\Min_{1\le\mu\le\nu\le M}\[m^2\(1-\cos{\theta_{\mu\nu}}\)\]
=m^2 \(1-\cos{\theta_{\min}}\),
\eea
where $\theta_{\min}\coloneqq \Min_{1\le\mu\le\nu\le M} \theta_{\mu\nu}$.
Then, it holds
\bea
m^2 \(1-\cos{\theta_{\min}}\) 
\ge 
\frac{1}{\beta}\ln(\frac{2(M-1)m}{R})+2mR.
\eea
\end{lemma}
\begin{proof}
This result directly follows from \cref{corollary:Delta_min} under \cref{assumption:patterns_on_sphere}.
\end{proof}

\begin{lemma}[\cite{ramsauer2020hopfield}]
\label{lemma:W}
Given the real numbers $a, b \in R$. While the equation
\bea
ac+c\ln{c}-b=0
\eea
holds, then we have the solution
\bea
c=\frac{b}{W_0(\exp(a+\ln{b}))}.
\eea
\end{lemma}
\begin{proof}
\bea
ac+c\ln(c)-b=0\\
a+\ln(c)=\frac{b}{c}\\
a+\ln(b)+\ln(\frac{c}{b})=\frac{b}{c}\\
\frac{b}{c}+\ln(\frac{b}{c})=a+\ln{b}\\
\frac{b}{c}\exp(\frac{b}{c})=\exp(a+\ln{b})\\
\frac{b}{c}=W_0(\exp{a+\ln{b}})\\
c=\frac{b}{W_0({\exp\{a+\ln{b}\}})}
\eea
\end{proof}

\begin{theorem}[Main Result: Memory Capacity of Sparse Hopfield]
\label{thm:memory_capacity}
Assume all memory patterns being on a sphere of radius $m$: $\norm{\bxi^\mu}=m$ for all $\mu$.
Let $1-p$ be the probability of successful retrieval.
\bea
M \ge \sqrt{p}C^\frac{d-1}{4},
\eea
when all patterns are randomly drawn from a $d$-dimensional sphere with radius $m$.
\end{theorem}
\begin{proof}[Proof Sketch]
The bound 
\end{proof}

\begin{proof}[Proof of \cref{thm:memory_capacity}]
From $\red{\Delta_\mu 
\ge
\frac{1}{\beta}\ln(\frac{2(M-1)m}{R})+2mR}$
, we can write down the probability of success storage and retrieval, i.e. minimal separation $\Delta_{\min}$ satisfies well-separation condition \cref{thm:well_separation}.

Let $\Delta_{\min}=\Min_{\mu\in[M]}\Delta_\mu$, and $\theta_{\mu\nu}$ be the angle between two patterns $\bxi^\mu$ and $\bxi^\nu$.
We have
\bea
\Delta_{\min}\ge 
\frac{1}{\beta}\ln(\frac{2(M-1)m}{R})+2mR,
\eea
and
\bea
\Delta_{\min}=\Min_{1\le\mu\le\nu\le M}\[m^2\(1-\cos{\theta_{\mu\nu}}\)\]
=m^2 \(1-\cos{\theta_{\min}}\),
\eea
where $\theta_{\min}\coloneqq \Min_{1\le\mu\le\nu\le M} \theta_{\mu\nu}\in[0,\pi]$.
Then, it holds
\bea
\label{eqn:cos}
m^2 \(1-\cos{\theta_{\min}}\) 
\ge 
\frac{1}{\beta}\ln(\frac{2(M-1)m}{R})+2mR.
\eea


With \cref{thm:well_separation}
, we write down the probability of success storage and retrieval
\bea
P\(\Delta_\mu\ge \frac{1}{\beta}\ln(\frac{2(M-1)m}{R})+2mR \)= 1-p.
\eea
By \eqref{eqn:cos}, we have
\bea
\label{success}
P\( m^2 \(1-\cos{\theta_{\min}}\) \ge  \frac{1}{\beta}\ln(\frac{2(M-1)m}{R})+2mR \) = 1-p.
\eea
By \cite[(4.22.2)]{olver2010nist}, for $0 \le \cos{\theta_{\min}} \le 1$, $\cos{\theta_{\min}}$ can be upper bounded by:
\bea
\cos{\theta_{\min}} \le 1- \frac{\theta_{\min}^2}{5}.
\eea
It holds
\bea
P\( \frac{m^2\theta_{\min}^2}{5} \ge \frac{1}{\beta}\ln(\frac{2(M-1)m}{R})+2mR\)= 1-p,
\eea
which can be rewritten as
\bea
P\(M^{\frac{2}{d-1}}\theta_{\min} \ge \frac{\sqrt{5}M^{\frac{2}{d-1}}}{m}\[\frac{1}{\beta}\ln(\frac{2(M-1)m}{R})+2mR\]^\half\) = 1-p.
\label{eqn:ineq1}
\eea
Here, $M^{\nicefrac{2}{d-1}}$ is introduced for later convenience.

Let 
\bea
\omega_d
\coloneqq 
\frac{2\pi^{\nicefrac{d+1}{2}}}{\Gamma\(\frac{d+1}{2}\)},
\eea
be the surface area of a $d$-dimensional unit sphere is, where $\Gamma(\cdot)$ represents the gamma function.

Intuitively, $\theta_{\mu,\nu}\in[0,\pi]$ represent the pairwise correlation of two patterns $\bxi_\mu$ and $\bxi_\nu$.
The probability distribution for $\theta\in[0,\pi]$ has been shown by \cite{cai2012phase} to be
\bea
\Red{
P(\theta)=\gamma_d\cdot \(1-\theta^2\)^{\frac{n-2}{2}},
}
\eea
where
\bea
\gamma_d \coloneqq \frac{1}{d} \frac{\omega_{d-1}}{\omega_d}=\frac{1}{d}\frac{\Gamma\(\frac{d+1}{2}\)}{\sqrt{\pi}\Gamma\(\frac{d}{2}\)}.
\eea

By \cite[Lemma~3.5]{brauchart2018random}, we obtain
\begin{align}
P&\(M^{\frac{2}{d-1}}\theta_{\min} \ge \frac{\sqrt{5}M^{\frac{2}{d-1}}}{m}\[\frac{1}{\beta}\ln(\frac{2(M-1)m}{R})+2mR\]^{\half}\)
= 1-p
\nonumber\\
&\quad\quad\quad\ge
1-\half\gamma_{d-1}5^{\frac{d-1}{2}}M^2 m^{-(d-1)}\[\frac{1}{\beta}\ln(\frac{2(M-1)m}{R})+2mR\]^{\frac{d-1}{2}},
\label{eqn:ineq2}
\end{align}
where $\gamma_d$ is defined as the ratio of surface areas of $(d-1)$- and $d$-dimensional unit sphere\footnote{Recall that, the surface area of a $d$-dimensional unit sphere is $\omega_d\coloneqq 2\pi^{(d+1)/2}/\Gamma\((d+1)/2\)$,  where $\Gamma(\cdot)$ represents the gamma function.}:
\bea
\gamma_d \coloneqq \frac{1}{d\sqrt{\pi}}\frac{\Gamma\(\frac{d+1}{2}\)}{\Gamma\(\frac{d}{2}\)}.
\eea
Recall $d, M\in \mathbb{N}_+$, $p\in [0,1]$. 
With some real value $C\in\R$, it holds
\bea
M=\sqrt{p}C^{\frac{d-1}{4}}.
\eea
Reformulating \eqref{eqn:ineq2}, we have
\bea
5^{\frac{d-1}{2}}
    \(\sqrt{p}C^{\frac{d-1}{4}}\)^2 m^{-(d-1)}\bigg\{\frac{1}{\beta}\ln{\[\frac{2(M-1)m}{R}\]}+\frac{1}{\beta}\bigg\}^{\frac{d-1}{2}}-p \le 0,
\eea
which leads to
\bea
5^{\frac{d-1}{2}}C^{\frac{d-1}{2}} m^{-(d-1)}\bigg\{\frac{1}{\beta}\ln{\[\frac{2(M-1)m}{R}\]}+\frac{1}{\beta}\bigg\}^{\frac{d-1}{2}}\le 1.
\label{eqn:ineq3}
\eea

To obtain the term like \cref{lemma:W}, we reformulate \ref{eqn:ineq3} as:
\bea
\frac{5c}{m^2}\bigg\{\frac{1}{\beta}+\frac{1}{\beta}\ln{\[2\beta m^2 \(pC^\frac{d-1}{2}-\sqrt{p}C^\frac{d-1}{4}\)\]}\bigg\}-1 \leq 0.
\eea
While we define
    \bea
    a\coloneqq \frac{2}{d-1} \{1+\ln{\[2\beta m^2\(p-\sqrt{p}C^{-\frac{d-1}{4}}\)\]} \}, b\coloneqq \frac{2\beta m^2}{5(d-1)},
    \eea
by lemma \ref{lemma:W}, we have the solution
\bea
C=\frac{b}{W_0({\exp\{a+\ln{b}\}})},
\eea
where $W_0$  is the upper branch of the Lambert $W$ function.
Since the domain of the Lambert $W$ function is $x>-\nicefrac{1}{e}$ and \red{the fact $\exp{a+\ln{b}}>0$}, the solution exists.

While $c$ fulfills inequality \ref{eqn:ineq3}, we obtain a lower bound on the exponential storage capacity $M$:
\bea
M
\geq
\sqrt{p}C^{\frac{d-1}{4}}
\eea

{\color{red}
To satisfy the well-separation condition, it is sufficient that (RHS of \eqref{eqn:ineq1} is lager than RHS of \eqref{eqn:ineq2}???)
\bea
\half\gamma_{d-1}5^{\frac{d-1}{2}}M^2 m^{-(d-1)}\[\frac{1}{\beta}\ln(\frac{2(M-1)m}{R})+2mR\]^{\frac{d-1}{2}}-p = 0.
\eea
}
\begin{itemize}
\color{firebrick}
    \item  

    Since $R\le R_{\text{Dense}}$, it holds
    \bea
    2mR \le 2mR_{\text{Dense}}=\frac{2}{\beta M} \le \frac{1}{\beta}.
    \eea

    \item 
    
    \item By the results of (\cite{olver2010nist},4.22), we have
    \bea
    \frac{\gamma_{d-1}}{2}\le \gamma_{d-1}\le 1.
    \eea
    \item
    We have
    \bea
    5^{\frac{d-1}{2}}
    \(\sqrt{p}C^{\frac{d-1}{4}}\)^2 m^{-(d-1)}\(\frac{1}{\beta}\ln(\frac{2(M-1)m}{R})+\frac{1}{\beta}\)^{\frac{d-1}{2}}-p \le 0,
    \eea
    which leads to
    \bea
    5^{\frac{d-1}{2}}
    C^{\frac{d-1}{2}} m^{-(d-1)}\(\frac{1}{\beta}\ln(\frac{2(M-1)m}{R})+\frac{1}{\beta}\)^{\frac{d-1}{2}}\le 1,
    \eea
    
    
    We have
    \bea
    ac + c\ln c -b \le 0.
    \eea
    \item
    \jhcomment{Should we set $m\coloneqq K \sqrt{d-1}$ with some $K\in \R$?}
    \bea
    5^{\frac{d-1}{2}}
    C^{\frac{d-1}{2}} \(\frac{1}{K^2(d-1)}\)^{\frac{d-1}{2}}\(\frac{1}{\beta}\ln(\frac{2(M-1)\(K \sqrt{d-1}\)}{R})+\frac{1}{\beta}\)^{\frac{d-1}{2}}\le 1,
    \eea
    and hence
    \bea
    \frac{5C}{K^2(d-1)}\(\frac{1}{\beta}\ln(\frac{2(M-1)\(K \sqrt{d-1}\)}{R})+\frac{1}{\beta}\)\le 1
    \eea

    \item Rearrange
    \bea
    \frac{5c}{m^2}\{\frac{1}{\beta}+\frac{1}{\beta}\ln{\[2\beta m^2 \(pC^\frac{d-1}{2}-\sqrt{p}C^\frac{d-1}{4}\)\]}\}-1 \leq 0\\
    \grey{
    \[\text{c.f.  }
    \frac{1}{\beta}\ln(\frac{2(M-1)m}{R})+\frac{1}{\beta}- \frac{m^2}{5C}
    \le0\]
    }
    \eea
    \item
    Define 
    \bea
    a\coloneqq 
    \frac{2}{d-1} \bigg\{1+\ln{\[2\beta m^2\(p-\sqrt{p}C^{-\frac{d-1}{4}}\)\]} \bigg\}
    , \quad
    b\coloneqq \frac{2\beta m^2}{5(d-1)}.
    \eea
    We have
    \bea
    ac + c\ln c -b \le 0.
    \eea
    
\end{itemize}
This inequality has the solution:
\bea
C=\frac{b}{W_0\(\exp{a+\ln b}\)},
\label{eqn:c}
\eea
where $W_0$  is the upper branch of the Lambert $W$ function.
Since the domain of the Lambert $W$ function is $x>-\nicefrac{1}{e}$ and \red{the fact $\exp{a+\ln{b}}>0$}, the solution exists.

While $c$ fulfills the master inequality, we obtain a lower bound on the exponential storage capacity $M$:
\bea
M
\geq
\sqrt{p}C^{\frac{d-1}{4}}
\eea


To compare with results from dense modern Hopfield, we denote the counterparts with $\Tilde{\cdot}$ notation, i.e. $\Tilde{a},\Tilde{b}$ for the dense version of $a,b$.

Comparing $a$ with the value of $\Tilde{a} \coloneqq \frac{2}{d-1} \[1+\ln{\(2\beta m^2 p\)}\]$ in \cite{ramsauer2020hopfield}, we have
\bea
\Tilde{a}
=
\frac{2}{d-1} \[1+\ln{\(2\beta m^2 p\)}\]
\geq
\frac{2}{d-1} \bigg\{1+\ln{\[2\beta m^2\(p-\sqrt{p}C^{-\frac{d-1}{4}}\)\]} \bigg\}
=
a.
\eea
, and therefore
\bea
W_0\(\exp{\Tilde{a}+\ln \Tilde{b}}\)
\geq
W_0\(\exp{a+\ln b}\).
\eea
Based on the solution of $C$ in \eqref{eqn:c}, we have
\bea
\Tilde{C} = \frac{b}{W_0\(\exp{\Tilde{a}+\ln \Tilde{b}}\)} \leq \frac{b}{W_0\(\exp\{a+\ln b\}\)} = C
\eea
Therefore, we obtain the capacity larger than that of \cite{ramsauer2020hopfield}
\bea
M=\sqrt{p}C^{\frac{d-1}{4}}
\geq
\sqrt{p}\Tilde{C}^{\frac{d-1}{4}}=\Tilde{M}.
\eea
\end{proof}
\begin{corollary}
The equality holds when $\norm{\bxi^\mu}=m$ for all $\mu$, i.e. when all memory patterns are on the sphere of radius $m$.
\end{corollary}





\begin{theorem}[Retrieval Accuracy Convergence Rate]
The convergence rate
\end{theorem}







==> retrieval_error_bounds.tex <==
Next, we introduce a theorem characterizing the retrieval error bound, assuming that the patterns follow a standard Gaussian distribution. Through the lens of such assumption, we elucidate the advantages of sparsity in comparison to the dense Hopfield model and identify the conditions under which these benefits arise.
\clearpage
\begin{theorem}[Retrieval Error Rates]
\label{thm:retrieval_error_rate}
Let $\calT_{\text{Dense}}$ be the retrieval dynamics of the dense modern Hopfield model \cite{ramsauer2020hopfield}.
Let $m\coloneqq \Max_{\mu\in[M]}\norm{\bxi_\mu}$, $n\coloneqq \norm{\bx}$ and $t\coloneqq  \abs{\sumM\Braket{\bxi_\mu,\bx}/M-2d}$.
Assume that the query pattern $\bx\in S_\mu$ and the set of memory patterns $\{\bxi_\nu\}_{\nu\in[M]}$ are i.i.d. samples drawn from $\bxi,\bx\sim N(0,\mathbf{1}_d)$.
Furthermore, suppose there exists an $\alpha > 0$ and sufficiently large $M$ and $d$ such that the following conditions hold: $\Braket{\bxi,\bx} \sim N(d, 2d)$, $\Max_{\nu\in[M]}{\Braket{\bxi_\nu,\bx}} = d + \alpha (2d)^{\nicefrac{1}{2}}$, $Mt^2/(nm)^2 \gg 1$, and $(1 + \alpha\sqrt{2/d})^{-M} \ll 1$.
Then, with high probability, it holds
\begin{align}
\norm{\calT_{\text{Dense}}\(\bx\)-\bxi^\mu}&\ge 
m\(d^{\nicefrac{1}{2}}\exp{\beta \alpha_2\(2d\)^{\nicefrac{1}{2}}}
-1
\)
\\
\norm{\calT\(\bx\)-\bxi^\mu}&\le
m+m\beta\(nmM+1\) 
+\beta mM \(d+\alpha_1(2d)^{\nicefrac{1}{2}}\).
\end{align}
\end{theorem}
Intuitively, the tighter error bound over dense models arises from the increased energy landscape separation provided by the sparse Hopfield energy function, which enables the separation of closely correlated patterns.
\begin{proof}[Proof Sketch]
Intuitively, the sparse retrieval error crucially depends on the
sparsity-dependent threshold element $\Braket{\bxi_\kappa,\bx}$ of the sparsemax function which provides the polynomial dependence in $d$.
On the other hand, all elements of softmax are outputs of exponentiation of $\Braket{\bxi_\kappa,\bx}$  which results to the exponential dependence in $d$.
\end{proof}

{\color{Blue}
We first introduce two auxiliary properties.
[Will move to appendix]
\begin{property}
\label{property:mean_convergence}
Let $m\coloneqq \Max_{\mu\in[M]}\norm{\bxi_\mu}$, $n\coloneqq \norm{\bx}$, and $\E\[\Braket{\bxi,\bx}\]\coloneqq \sum_\nu^M \Braket{\bxi_{\nu},\bx}$ be the empirical mean of $\{\Braket{\bxi_1,\bx},\ldots,\Braket{\bxi_M,\bx}\}$.
Assume $\Braket{\bxi,\bx}\sim N(\mu,\sigma^2)$.
With at least probability $1-2\exp{-\frac{2Mt^2}{(2nm)^2}}$, it holds
\bea
\mu-t \le \E\[\Braket{\bxi,\bx}\]\le \mu +t,
\eea
where $t\coloneqq  \abs{\E\[\Braket{\bxi,\bx}\]-\mu}$.
\end{property}
\begin{proof}[Proof of Convergence of Empirical Mean and True Mean]
Let $\E\[\Braket{\bxi,\bx}\]$ be the empirical mean of of the sample of size $M$, $\{\Braket{\bxi_1,\bx},\ldots,\Braket{\bxi_M,\bx}\}$ and bounded in the interval $[-nm, nm]$.
By Hoeffding's inequality, we have
\bea
P\(\abs{\E\[\Braket{\bxi,\bx}\]-\mu}\le t \)
\le 2\exp{-\frac{2Mt^2}{(2nm)^2}}.
\eea
Then, let $\delta = 2\exp{-\frac{2Mt^2}{(2nm)^2}}$, with at least probability $1-\delta$, we have
\bea
\mu-t \le \E\[\Braket{\bxi,\bx}\]\le \mu +t,
\eea
where $t\coloneqq  \abs{\E\[\Braket{\bxi,\bx}\]-\mu}$.
\end{proof}
\begin{property}
\label{property:greater_than_mu_sigma}
Given $\Braket{\bxi,\bx}\sim N(\mu,\sigma)$, and a set of samples of size M, $\{\Braket{\bxi_1,\bx},\ldots, \Braket{\bxi_M,\bx}\}$.
With at least $1-\(\frac{\mu}{\mu+\alpha\sigma}\)^M$ probability, we have
\bea
\Max_{\nu\in[M]}\Braket{\bxi_\nu,\bx}>\mu+\alpha\sigma.
\eea
Therefore, with at least the same probability, there exists a $\alpha'>\alpha$ such that
\bea
\Max_{\nu\in[M]}\Braket{\bxi_\nu,\bx}=\mu+\alpha'\sigma
\eea
\end{property}
\begin{proof}[Proof]
Given $\Braket{\bxi,\bx}\sim N(\mu,\sigma)$, and a set of samples of size M, $\{\Braket{\bxi_1,\bx},\ldots, \Braket{\bxi_M,\bx}\}$.
\bea
P\(\Max_{\nu\in[M]}\Braket{\bxi_\nu,\bx}>\mu+\alpha_2\sigma\)=
1- P\(\Max_{\nu\in[M]}\Braket{\bxi_\nu,\bx}\le \mu+\alpha_2\sigma\).
\eea
Since all samples are iid drawn, we have
\begin{align}
P\(\Max_{\nu\in[M]}\Braket{\bxi_\nu,\bx}\le \mu+\alpha_2\sigma\)
=
\prod_{\nu=1}^M P\(\Braket{\bxi_\nu,\bx}\le \mu+\alpha_2\sigma\),
\end{align}
Note that
\begin{align}
P\(\Braket{\bxi_\nu,\bx}\le \mu+\alpha_2\sigma\)
&=P\(-\Braket{\bxi_\nu,\bx}\ge -(\mu+\alpha_2\sigma)\)\\
&\le
\frac{\mu}{\mu+\alpha_2\sigma}
\annot{By Markov inequality},
\end{align}
we have
\begin{align}
P\(\Max_{\nu\in[M]}\Braket{\bxi_\nu,\bx}>\mu+\alpha_2\sigma\)\ge 
1- \(\frac{\mu}{\mu+\alpha_2\sigma}\)^M.
\end{align}
\end{proof}
}
\begin{proof}[Proof of \cref{thm:retrieval_error_rate}]
Recall
\bea
\bz = \beta \bm{\bm{\Xi}}^\sT\bx = \beta \(\Braket{\bxi_1,\bx},\ldots, \Braket{\bxi_M,\bx}\),
\eea
with 
$
z_\mu =\beta \Braket{\bxi_\mu,\bx}.
$
{\color{red}
[The assumptions on distribution are wrong.]
Since $\bxi,\bx \sim N(0,\mathbf{1}_d)$, the distribution of $\Braket{\bxi,\bx}$ is given by
\bea
\Braket{\bxi,\bx}\sim \chi^2(d),
\eea
where  $\chi^2(d)$ is the chi-square distribution with degrees of freedom $d$.
By central limit theorem under large $d$ limit, it can be approximated as
\bea
\Braket{\bxi,\bx}\sim N\(d,2d\).
\eea
Hence, we have
\bea
z = \beta \Braket{\bxi,\bx}  \sim N\(\beta d,2\beta^2d\).
\eea
}

We first provide an upper bound of the sparse retrieval error for a query $\bx\in S_\mu$ given memory patterns $\{\bxi_\nu\}_{\nu\in[M]}$.

According to the definition of sparsemax (\cref{lemma:sparsemax_exact}), it holds
\begin{align}
[ \Sparsemax \(\beta \bm{\Xi}^\sT \bx\) ]_\mu 
&\le 
\[\beta \bm{\Xi}^\sT \bx \]_{\mu}-\[\beta \bm{\Xi}^\sT \bx\]_{(\kappa)}+\frac{1}{\kappa},
\label{eqn:sparsemax_upper_identity}
\end{align}
for all $\mu\in[M]$.
Then, the sparse retrieval error is given as
\begin{align}
\norm{\calT\(\bx\)-\bxi^\mu}&=
\norm{\bm{\bm{\Xi}}\Sparsemax\(\beta \bm{\bm{\Xi}}^\sT \bx\)-\bxi^\mu}
=\norm{\sum_{\nu=1}^{\kappa} \bxi_{(\nu)} \[\Sparsemax\(\beta \bm{\bm{\Xi}}^\sT \bx\) \]_{(\nu)}-\bxi^\mu}\nonumber\\
&\le 
m+m\beta \norm{\sum^{\kappa}_{\nu=1} \(\[ \bm{\Xi}^\sT \bx \]_{(\nu)}-\[ \bm{\Xi}^\sT \bx\]_{(\kappa)}+\frac{1}{\beta\kappa}\)\frac{\bxi_{(\nu)}}{m}}
\annot{By \eqref{eqn:sparsemax_upper_identity}}\\
&\le 
m+m\beta \norm{\sum^{\kappa}_{\nu=1}\( \[ \bm{\Xi}^\sT \bx \]_{(\nu)}-\[ \bm{\Xi}^\sT \bx\]_{(\kappa)}+\frac{1}{\beta\kappa}\)\bI_d}
\\
&=
m+d^{\nicefrac{1}{2}}m\beta \abs{\sum^{\kappa}_{\nu=1}\( \[ \bm{\Xi}^\sT \bx \]_{(\nu)}-\[ \bm{\Xi}^\sT \bx\]_{(\kappa)}+\frac{1}{\beta\kappa}\)}
\\
&= 
m+d^{\nicefrac{1}{2}}m\beta \[\sum^{\kappa}_{\nu=1}\( \[ \bm{\Xi}^\sT \bx \]_{(\nu)}-\[ \bm{\Xi}^\sT \bx\]_{(\kappa)}+\frac{1}{\beta\kappa}\)\]
\\
&\le 
m+d^{\nicefrac{1}{2}}m\beta \[\kappa \(\Max_{\nu\in[M]}\Braket{\bxi_\nu,\bx}-\[ \bm{\Xi}^\sT \bx\]_{(\kappa)}\)+\frac{1}{\beta}\]
\\
&\le 
m+d^{\nicefrac{1}{2}}m\beta \[\kappa \(nm-\[ \bm{\Xi}^\sT \bx\]_{(\kappa)}\)+\frac{1}{\beta}\]
\\
&=
m+d^{\nicefrac{1}{2}}nm^2\beta \[\kappa \(1-\frac{\[ \bm{\Xi}^\sT \bx\]_{(\kappa)}}{nm}\)+\frac{1}{\beta nm}\]
\end{align}


Similarly, we provide a lower bound of the dense retrieval error.
Let $t\coloneqq \abs{\E\[\Braket{\bxi,\bx}\]-\mu}$ with $\E\[\Braket{\bxi,\bx}\]$ and $\mu$ being the empirical mean and true mean of $\Braket{\bxi,\bx}$, we have
\begin{align}
    \norm{\calT_{\text{Dense}}(\bx)-\bxi_\mu}
    &=
\norm{\bxi_\mu-\sum^M_{\nu=1} [\Softmax(\beta \bm{\Xi}^\sT \bx)]_\nu \bxi_\nu}\\
&\ge
\norm{\bx_\mu^\star-\bxi_\mu}
\end{align}

{\color{firebrick}
\begin{align}
\norm{\calT_{\text{Dense}}-\bxi_\mu}
-\norm{\calT-\bxi_\mu}
&\ge 
\norm{\calT_{\text{Dense}}}-\norm{\calT}\\
&=
\norm{\sum^M_{\nu=1} [\Softmax\(\beta \bm{\Xi}^\sT \bx\)]_\nu \bxi_\nu}
-\norm{\sum^M_{\nu=1} [\Sparsemax\(\beta \bm{\Xi}^\sT \bx\)]_\nu \bxi_\nu}\\
&=
\norm{\sum^M_{\nu=1} [\Softmax\(\beta \bm{\Xi}^\sT \bx\)]_\nu \bxi_\nu}
-\norm{\sum^\kappa_{\nu=1} [\Sparsemax\(\beta \bm{\Xi}^\sT \bx\)]_\nu \bxi_\nu}
\end{align}


Let 
\bea
\bm{\Xi}^\sT \bx\coloneqq \(\underbrace{Y,\ldots,Y}_{\kappa},\underbrace{y,\ldots,y}_{d-\kappa}\),
\eea
with $\kappa+(d-\kappa)=d$
such that
\bea
\Sparsemax\(\bm{\Xi}^\sT \bx\)
=
\(\underbrace{\Tilde{Y},\ldots,\Tilde{Y}}_{\kappa},\underbrace{0,\ldots,0}_{d-\kappa}\),
\eea
where $\kappa$ is the intrinsic dimension (sparsity) and $\Tilde{Y}=\frac{1}{\kappa}$.
}


\clearpage
{\color{black!50}
Similarly, we provide a lower bound of the dense retrieval error:
\begin{align}
    \norm{\calT_{\text{Dense}}(\bx)-\bxi_\mu}
    &=
\norm{\bxi_\mu-\sum^M_{\nu=1} [\Softmax(\beta \bm{\Xi}^\sT \bx)]_\nu \bxi_\nu}\\
&\ge 
\norm{\bxi_\mu-mM \Softmax\(\beta \Max_{\nu\in [M]}\Braket{\bxi_\nu,\bx}\)\mathbf{1}_d}\\
&\ge 
\norm{\bxi_\mu-mM 
\frac{\exp{\beta \Max_{\nu\in [M]}\Braket{\bxi_\nu,\bx}}}{M \sumM \exp{\beta \Braket{\bxi_\mu,\bx} }}
\mathbf{1}_d
}
\annot{$\E\[e^X\]\ge e^{\E\[X\]}$}
\\
&\ge 
\norm{\bxi_\mu-mM 
\frac{\exp{\beta \Max_{\nu\in [M]}\Braket{\bxi_\nu,\bx}}}{M \exp{\beta d }}
\mathbf{1}_d
}
\annot{With high probability, by \cref{property:mean_convergence}}\\
&\ge 
m\(
d^{\nicefrac{1}{2}}\abs{\frac{\exp{\beta \Max_{\nu\in [M]}\Braket{\bxi_\nu,\bx}}}{ \exp{\beta d }}}
-\norm{\frac{\bxi_\mu}{m}}
\)\\
&\ge 
m\(d^{\nicefrac{1}{2}}\exp{\beta {\Max_{\nu\in [M]}\Braket{\bxi_\nu,\bx}-\beta d}}
-1
\)
\annot{$m=\Max_{\nu\in[M]}\bxi_\nu$}
\\
&=
m\(d^{\nicefrac{1}{2}}\exp{\beta \alpha\(2d\)^{\nicefrac{1}{2}}}
-1
\), \quad\text{for some } \alpha\ge 0.
\annot{With high probability, by \cref{property:greater_than_mu_sigma}}
\end{align}}


\end{proof}





\clearpage
\begin{theorem}[Retrieval Error Rates]
\label{thm:retrieval_error_rate}
Under large $d$ and $M\gg d$ limits.
Assume $\bx\sim N(0,\mathbf{1}_d)$ and $\bxi\sim N(0,\mathbf{1}_d)$. For some $\alpha_1,\alpha_2\ge 0.$
\begin{align}
\norm{\calT_{\text{Dense}}\(\bx\)-\bxi^\mu}&\ge 
m\(d^{\nicefrac{1}{2}}\exp{\beta \alpha_2\[\frac{d\beta^2}{2}\]^{\nicefrac{1}{2}}}
-1
\)
=\calO(d^{\nicefrac{1}{2}}e^{d^{\nicefrac{1}{2}}})
\\
\norm{\calT\(\bx\)-\bxi^\mu}&\le
m+m\beta\(nmM+1\) 
+\half\beta mM \abs{d+\alpha_1\sqrt{\half d}}=\calO(d).
\end{align}
\end{theorem}
\begin{proof}[Proof of \cref{thm:retrieval_error_rate}]
Take large $d$ and $M\gg d$ limits.
Let $\bx\sim N(0,\mathbf{1}_d)$ and 
$\bxi\sim N(0,\mathbf{1}_d)$.


Recall
\bea
\bz = \beta \bm{\bm{\Xi}}^\sT\bx = \beta \(\Braket{\bxi_1,\bx},\ldots, \Braket{\bxi_M,\bx}\),
\eea
with
\bea
z_\mu =\beta \Braket{\bxi_\mu,\bx},
\eea




Therefore, denoting  $\chi^2(d)$ is the chi-square distribution with degrees of freedom $d$,
\bea
\Braket{\bxi,\bx}\sim \chi^2(d),
\eea
which, by central limit theorem under large $d$ limit, is
\bea
\Braket{\bxi,\bx}\sim N\(d,2d\).\quad
\grey{\[\text{c.f }\Braket{\bxi,\bxi}\sim N\(d,2d\)\]}
\eea

Hence
\bea
z = \beta \Braket{\bxi,\bx}  \sim N\(\beta d,2\beta^2d\).
\eea



\clearpage
\begin{mdframed}
\begin{proof}[Convergence of Empirical Mean and True Mean]
Let $\E\[\Braket{\bxi,\bx}\]$ be the empirical mean of of the sample of size $M$, $\{\Braket{\bxi_1,\bx},\ldots,\Braket{\bxi_M,\bx}\}$ and bounded in the interval $[-nm, nm]$.
By Hoeffding's inequality, we have
\bea
P\(\abs{\E\[\Braket{\bxi,\bx}\]-\mu}\le t \)
\le 2\exp{-\frac{2Mt^2}{(2nm)^2}}.
\eea
Then, let $\delta = 2\exp{-\frac{2Mt^2}{(2nm)^2}}$, with at least probability $1-\delta$, we have
\bea
\mu-t \le \E\[\Braket{\bxi,\bx}\]\le \mu +t.
\eea
Therefore, for $\delta\ll 1$, we need
\bea
M\gg 2\(\frac{nm}{t}\)^2,
\eea
where $t\coloneqq  \abs{\E\[\Braket{\bxi,\bx}\]-\mu}$.
\end{proof}
\end{mdframed}

\begin{mdframed}
\begin{claim}
\begin{property}
\label{property:greater_than_mu_sigma}
Given $\Braket{\bxi,\bx}\sim N(\mu,\sigma)$, and a set of samples of size M, $\{\Braket{\bxi_1,\bx},\ldots, \Braket{\bxi_M,\bx}\}$.
With at least $1-\(\frac{\mu}{\mu+\alpha\sigma}\)^M$ probability, we have
\bea
\Max_{\nu\in[M]}\Braket{\bxi_\nu,\bx}>\mu+\alpha\sigma.
\eea
Therefore, with at least the same probability, there exists a $\alpha'>\alpha$ such that
\bea
\Max_{\nu\in[M]}\Braket{\bxi_\nu,\bx}=\mu+\alpha'\sigma
\eea
Furthermore, by setting $\Braket{\bxi_{\kappa},\bx}\coloneqq \mu+\alpha_3\sigma$, we have
\bea
\Max_{\nu\in[M]}\Braket{\bxi_\nu,\bx}>\Braket{\bxi_{\kappa},\bx},
\eea
with at least $1-\(\frac{\mu}{\mu+\alpha_3\sigma}\)^M$ probability.
For $\mu= d $ and $\sigma=(2d)^{\nicefrac{1}{2}}$, we have
\bea
\(\frac{\mu}{\mu+\alpha\sigma}\)^M
=
\(\frac{d}{d+\alpha (2d)^{\nicefrac{1}{2}}}\)^M \sim \calO()
\eea
\end{property}
\end{claim}
\begin{proof}[Another Proof]
Given $\Braket{\bxi,\bx}\sim N(\mu,\sigma)$, and a set of samples of size M, $\{\Braket{\bxi_1,\bx},\ldots, \Braket{\bxi_M,\bx}\}$.
\bea
P\(\Max_{\nu\in[M]}\Braket{\bxi_\nu,\bx}>\mu+\alpha_2\sigma\)=
1- P\(\Max_{\nu\in[M]}\Braket{\bxi_\nu,\bx}\le \mu+\alpha_2\sigma\).
\eea
Since all samples are iid drawn, we have
\begin{align}
P\(\Max_{\nu\in[M]}\Braket{\bxi_\nu,\bx}\le \mu+\alpha_2\sigma\)
=
\prod_{\nu=1}^M P\(\Braket{\bxi_\nu,\bx}\le \mu+\alpha_2\sigma\),
\end{align}
Note that
\begin{align}
P\(\Braket{\bxi_\nu,\bx}\le \mu+\alpha_2\sigma\)
&=P\(-\Braket{\bxi_\nu,\bx}\ge -(\mu+\alpha_2\sigma)\)\\
&\le
\frac{\mu}{\mu+\alpha_2\sigma}
\annot{By Markov inequality},
\end{align}
we have
\begin{align}
P\(\Max_{\nu\in[M]}\Braket{\bxi_\nu,\bx}>\mu+\alpha_2\sigma\)\ge 
1- \(\frac{\mu}{\mu+\alpha_2\sigma}\)^M.
\end{align}
{\color{firebrick}
Can we write
\bea
\Max_{\nu\in[M]}\Braket{\bxi_\nu,\bx}= \mu+\alpha_2\sigma + \(\cdots\)
\eea
?
}
\end{proof}
\end{mdframed}


\begin{claim}
According to the definition of sparsemax, we have
\begin{align}
[ \Sparsemax \(\beta \bm{\Xi}^\sT \bx\) ]_\mu &=\[\beta \bm{\Xi}^\sT \bx \]_{\mu}+\frac{1-\sum_{\nu \leq \kappa} \[\beta \bm{\Xi}^\sT \bx\]_{(\nu)}}{\kappa}\\
&\le 
\[\beta \bm{\Xi}^\sT \bx \]_{\mu}-\[\beta \bm{\Xi}^\sT \bx\]_{(\kappa)}+\frac{1}{\kappa}.
\label{eqn:sparsemax_upper_identity}
\end{align}

Then, the sparse retrieval error is given as
    \begin{align}
\norm{\calT\(\bx\)-\bxi^\mu}&=
\norm{\bm{\bm{\Xi}}\Sparsemax\(\beta \bm{\bm{\Xi}}^\sT \bx\)-\bxi^\mu}
=
\norm{\sum_{\nu=1}^{\kappa} \bxi^\nu \[\Sparsemax\(\beta \bm{\bm{\Xi}}^\sT \bx\) \]_\nu-\bxi^\mu}\nonumber\\
&\leq \norm{\bxi^\mu}+\norm{\sum^{\kappa}_{\nu=1} \[ \Sparsemax(\beta \bm{\bm{\Xi}}^T x)\]_\nu \bxi^\nu}\\
&\le 
m+m\beta \norm{\sum^{\kappa}_{\nu=1} \[ \bm{\Xi}^\sT \bx \]_{\nu}-\kappa\[ \bm{\Xi}^\sT \bx\]_{(\kappa)}+1}
\annot{By \eqref{eqn:sparsemax_upper_identity}}
\\
&\le 
m+m\beta \norm{\sum^{M}_{\nu=1} \[ \bm{\Xi}^\sT \bx \]_{\nu}-\kappa\[ \bm{\Xi}^\sT \bx\]_{(\kappa)}+1}\\
&\le 
m+m\beta \norm{nmM-\kappa\[ \bm{\Xi}^\sT \bx\]_{(\kappa)}+1}\\
&\le 
m+m\beta \(\norm{nmM+1}+\norm{\kappa\[ \bm{\Xi}^\sT \bx\]_{(\kappa)}}\)\\
&\le
m+m\beta\(nmM+1\) 
+\beta mM \abs{\[ \bm{\Xi}^\sT \bx\]_{(\kappa)}}
\annot{$M>\kappa$}
\\
&\le
m+m\beta\(nmM+1\) 
+\half\beta mM \red{\abs{\Max_{\nu\in[M]}\[ \bm{\Xi}^\sT \bx\]_{(\nu)}}}
\annot{$\Max_{\nu\in[M]}\[ \bm{\Xi}^\sT \bx\]_{(\nu)}>\[ \bm{\Xi}^\sT \bx\]_{(\kappa)}$}
\\
&=
m+m\beta\(nmM+1\) 
+\half\beta mM \red{\abs{\mu+\alpha_1\sigma}},
\quad \text{for } \alpha_1\ge 0,
\annot{$M\gg d$, with high probability}\\
&=
m+m\beta\(nmM+1\) 
+\half\beta mM \abs{d+\alpha_1\sqrt{\half d}},
\quad \text{for } \alpha_1\ge 0,
\end{align}
\end{claim}




On the other hand
\jhcomment{Old. Might be wrong.}
\begin{claim}
\begin{align}
    \norm{\calT_{\text{Dense}}(\bx)-\bxi_\mu}
    &=
\norm{\bxi_\mu-\sum^M_{\nu=1} [\Softmax(\beta \bm{\Xi}^\sT \bx)]_\nu \bxi_\nu}\\
&\ge 
\norm{\bxi_\mu-mM \Softmax\(\beta \Max_{\mu\in [M]}\Braket{\bxi_\mu,\bx}\)\mathbf{1}_d}\\
&= 
\norm{\bxi_\mu-mM 
\frac{\exp{\beta \Max_{\mu\in [M]}\Braket{\bxi_\mu,\bx}}}{\sum_{\nu}^M \exp{\beta \Braket{\bxi_\nu,\bx}}}
\mathbf{1}_d}\\
&=
\norm{\bxi_\mu-mM 
\frac{\exp{\beta \Max_{\mu\in [M]}\Braket{\bxi_\mu,\bx}}}{M \exp{\beta^2d }}
\mathbf{1}_d
}
\annot{$M\gg d$}\\
&=
m\norm{\frac{\exp{\beta \Max_{\mu\in [M]}\Braket{\bxi_\mu,\bx}}}{ \exp{\beta^2d }}\mathbf{1}_d-
\frac{\bxi_\mu}{m}
}\\
&\ge 
m\(
d^{\nicefrac{1}{2}}\abs{\frac{\exp{\beta \Max_{\mu\in [M]}\Braket{\bxi_\mu,\bx}}}{ \exp{\beta^2 d }}}
-\norm{\frac{\bxi_\mu}{m}}
\)
\\
&\ge 
m\(d^{\nicefrac{1}{2}}\exp{\beta \red{\Max_{\mu\in [M]}\Braket{\bxi_\mu,\bx}-\beta^2d}}
-1
\)\\
&=
m\(d^{\nicefrac{1}{2}}\exp{\beta \red{\alpha_2\sigma}}
-1
\), \quad\text{for some } \alpha_2\ge 0
\annot{Under $M\gg d$ \& $X\sim N(\mu,\sigma^2)$, then, with high probability, $\Max X=\mu+\alpha \sigma$ for some $\alpha\ge 0$}
\\
&=
m\(d^{\nicefrac{1}{2}}\exp{\beta \alpha_2\[\frac{d\beta^2}{2}\]^{\nicefrac{1}{2}}}
-1
\)
\end{align}
\end{claim}
\end{proof}


\clearpage
{\color{firebrick}
\textbf{TODO}:
Given 
\bea
\norm{\calT_{\text{Dense}}(\bx)-\bxi_\mu}\le 2m(M-1)\exp{-\beta m^2 \(1-\Max_{\nu,\nu\neq \mu }\Braket{\bxi_\mu,\bxi_\nu}\)}.
\eea
\begin{proof}
To link $\Delta_\mu$ to $\calT$, we first bound $\epsilon_{\text{Dense}}$ via \cite[Lemma~A.4]{ramsauer2020hopfield}:
\begin{align}
\epsilon_{\text{Dense}}&=\norm{\calT_{\text{Dense}}(\bx)-\bxi_\mu}\\
&=
\norm{\bxi_\mu-\sum^M_{\nu=1} [\Softmax(\beta \bm{\Xi}^\sT \bx)]_\nu \bxi_\nu}\\
&=
\norm{\(1-\[\Softmax(\beta \bm{\Xi}^\sT \bx)\]_\mu\)\bxi_\mu-\sum^M_{\nu=1, \nu \neq \mu}\[\Softmax(\beta \bm{\Xi}^\sT \bx)\]_\nu\bxi_\nu}\\
&\leq
\tilde{\epsilon} \norm{\bxi_\mu}+\frac{\tilde{\epsilon}}{M-1}\sum^M_{\nu=1, \nu \neq \mu} \norm{\bxi_\nu}\\
&\le 
\tilde{\epsilon} \( m+\frac{1}{M-1}\sum^M_{\nu=1, \nu \neq \mu} m\)
\\
\label{eqn:bound_eps}
&\leq
2\tilde{\epsilon} m,
\end{align}
where $\tilde{\epsilon}\coloneqq (M-1)\exp{-\beta \tilde{\Delta}_\mu}$ and the inequality 
\bea
\[\Softmax(\beta \bm{\Xi}^\sT \bx)\]_\nu
=\frac{\exp{\beta\(\Braket{\bx,\bxi_\nu}-\Braket{\bx,\bxi_\mu}\)}}{1+\sum_{\nu'\neq \mu} \exp{\beta\(\Braket{\bx,\bxi_{\nu'}}-\Braket{\bx,\bxi_\mu}\)}}
\le 
\exp{-\beta \Tilde{\Delta}_\mu},
\eea is used in the fourth line.
\end{proof}
\begin{enumerate}
    \item Construct a lower bound of $\norm{\calT_{\text{Dense}}-\bxi_\mu}$, say $L_{\text{Dense}}$.

    \item Construct a upper bound of $\norm{\calT-\bxi_\mu}$, say $U_{\text{Sparse}}$

    \item Show that
    \bea
    U_{\text{Sparse}} \le L_{\text{Dense}},
    \eea
    such that the sparse retrieval error is in general tighter.

    \item Also identify conditions for above failed to hold.
\end{enumerate}
}
\begin{proof}[\red{Wrong!}]
Take large $d$ and $M\gg d$ limits.
Let $\bx\sim N(0,\mathbf{1}_d)$ and $\by\sim N(0,\mathbf{1}_d)$.
For simplicity of presentation, we set 
\red{$\bxi\coloneqq \by\sim N(0,\mathbf{1}_d)$ [Returns out we don't need to multiple $m$.]}


Recall
\bea
\bz = \beta \bm{\bm{\Xi}}^\sT\bx = \beta \(\Braket{\bxi_1,\bx},\ldots, \Braket{\bxi_M,\bx}\),
\eea
such that 
\bea
z_\mu =\beta \Braket{\bxi_\mu,\bx},
\eea


\bea
xy \sim \frac{\Var(x+y)}{4} \chi + \frac{\Var(x-y)}{4} \chi
=\half \chi^2(1),
\eea
where $\chi^2(1)$ is the chi-square distribution with degrees of freedom one.


Therefore,
\bea
\Braket{\bxi,\bx}\sim \half\chi^2(d),
\eea
which, under large $d$ limit is
\bea
\Braket{\bxi,\bx}\sim N\(d,\frac{d}{2}\).\quad
\grey{\[\text{c.f }\Braket{\bxi,\bxi}\sim N\(d,\frac{d}{2}\)\]}
\eea
Hence
\bea
z = \beta \Braket{\bxi,\bx}  \sim N\(\beta d,\frac{d\beta^2}{2}\).
\eea

\begin{claim}
\begin{align}
[ \Sparsemax \(\beta \bm{\Xi}^\sT \bx\) ]_\mu &=\[\beta \bm{\Xi}^\sT \bx \]_{\mu}+\frac{1-\sum_{\nu \leq \kappa} \[\beta \bm{\Xi}^\sT \bx\]_{(\nu)}}{\kappa}\\
&\le 
\[\beta \bm{\Xi}^\sT \bx \]_{\mu}-\[\beta \bm{\Xi}^\sT \bx\]_{(\kappa)}+\frac{1}{\kappa}
\end{align}
    Given 
    \begin{align}
\norm{\calT\(\bx\)-\bxi^\mu}&=
\norm{\bm{\bm{\Xi}}\Sparsemax\(\beta \bm{\bm{\Xi}}^\sT \bx\)-\bxi^\mu}
=
\norm{\sum_{\nu=1}^{\kappa} \bxi^\nu \[\Sparsemax\(\beta \bm{\bm{\Xi}}^\sT \bx\) \]_\nu-\bxi^\mu}\nonumber\\
&\leq \norm{\bxi^\mu}+\norm{\sum^{\kappa}_{\nu=1} \[ \Sparsemax(\beta \bm{\bm{\Xi}}^T x)\]_\nu \bxi^\nu}\\
&\leq 
m+\kappa\abs{\frac{\Max_{\nu\in[\kappa]}\[\beta \bm{\bm{\Xi}}^\sT \bx \]_{\nu}}{\kappa}}m\\
&= 
\(1+\abs{\[\beta \bm{\bm{\Xi}}^\sT \bx \]_{\kappa}}\)m\\
&\le
m\(1+\beta \abs{\mu+\alpha_1\sigma}\)
=
m\[1+\beta \(\beta d+\alpha_1\(\frac{d\beta^2}{2}\)^{\nicefrac{1}{2}}\)\],
\quad \text{for } \alpha_1\ge 0,
\\
&
\red{
\le 
m\(1+ \beta \abs{\Max_{\mu\in [M]}\Braket{\bxi_\mu,\bx}}\)
}
.
\end{align}
\end{claim}
\begin{claim}
    On the other hand
\begin{align}
    \norm{\calT_{\text{Dense}}(\bx)-\bxi_\mu}
    &=
\norm{\bxi_\mu-\sum^M_{\nu=1} [\Softmax(\beta \bm{\Xi}^\sT \bx)]_\nu \bxi_\nu}\\
&\ge 
\norm{\bxi_\mu-mM \Softmax\(\beta \Max_{\mu\in [M]}\Braket{\bxi_\mu,\bx}\)\mathbf{1}_d}\\
&= 
\norm{\bxi_\mu-mM 
\frac{\exp{\beta \Max_{\mu\in [M]}\Braket{\bxi_\mu,\bx}}}{\sum_{\nu}^M \exp{\beta \Braket{\bxi_\nu,\bx}}}
\mathbf{1}_d}\\
&=
\norm{\bxi_\mu-mM 
\frac{\exp{\beta \Max_{\mu\in [M]}\Braket{\bxi_\mu,\bx}}}{M \exp{\beta^2d }}
\mathbf{1}_d
}
\annot{$M\gg d$}\\
&=
m\norm{\frac{\exp{\beta \Max_{\mu\in [M]}\Braket{\bxi_\mu,\bx}}}{ \exp{\beta^2d }}\mathbf{1}_d-
\frac{\bxi_\mu}{m}
}\\
&\ge 
m\(
d^{\nicefrac{1}{2}}\abs{\frac{\exp{\beta \Max_{\mu\in [M]}\Braket{\bxi_\mu,\bx}}}{ \exp{\beta^2 d }}}
-\norm{\frac{\bxi_\mu}{m}}
\)
\\
&\ge 
m\(d^{\nicefrac{1}{2}}\exp{\beta \red{\Max_{\mu\in [M]}\Braket{\bxi_\mu,\bx}-\beta^2d}}
-1
\)\\
&=
m\(d^{\nicefrac{1}{2}}\exp{\beta \red{\alpha_2\sigma}}
-1
\), \quad\text{for some } \alpha_2\ge 0
\annot{Under $M\gg d$ \& $X\sim N(\mu,\sigma^2)$, then $\Max X=\mu+\alpha \sigma$ for some $\alpha\ge 0$}
\\
&=
m\(d^{\nicefrac{1}{2}}\exp{\beta \alpha_2\[\frac{d\beta^2}{2}\]^{\nicefrac{1}{2}}}
-1
\)
\end{align}
\end{claim}
{\color{firebrick}
\begin{claim}
    On the other hand
\begin{align}
    \norm{\calT_{\text{Dense}}(\bx)-\bxi_\mu}
    &=
\norm{\bxi_\mu-\sum^M_{\nu=1} [\Softmax(\beta \bm{\Xi}^\sT \bx)]_\nu \bxi_\nu}\\
&\ge 
\norm{\bxi_\mu-mM \Softmax\(\beta \Max_{\mu\in [M]}\Braket{\bxi_\mu,\bx}\)\mathbf{1}_d}\\
&= 
\norm{\bxi_\mu-mM 
\frac{\exp{\beta \Max_{\mu\in [M]}\Braket{\bxi_\mu,\bx}}}{\sum_{\nu}^M \exp{\beta \Braket{\bxi_\nu,\bx}}}
\mathbf{1}_d}\\
&=
\norm{\bxi_\mu-mM 
\frac{\exp{\beta \Max_{\mu\in [M]}\Braket{\bxi_\mu,\bx}}}{M \exp{\beta^2d }}
\mathbf{1}_d
}
\annot{$M\gg d$}\\
&=
m\norm{\frac{\exp{\beta \Max_{\mu\in [M]}\Braket{\bxi_\mu,\bx}}}{ \exp{\beta^2d }}\mathbf{1}_d-
\frac{\bxi_\mu}{m}
}\\
&\ge 
m\(
d^{\nicefrac{1}{2}}\abs{\frac{\exp{\beta \Max_{\mu\in [M]}\Braket{\bxi_\mu,\bx}}}{ \exp{\beta^2 d }}}
-\norm{\frac{\bxi_\mu}{m}}
\)
\\
&\ge 
m\(d^{\nicefrac{1}{2}}\exp{\beta \red{\Max_{\mu\in [M]}\Braket{\bxi_\mu,\bx}-\beta^2d}}
-1
\)\\
&=
m\(d^{\nicefrac{1}{2}}\exp{\beta \red{\alpha_2\sigma}}
-1
\), \quad\text{for some } \alpha_2\ge 0
\annot{Under $M\gg d$ \& $X\sim N(\mu,\sigma^2)$, then $\Max X=\mu+\alpha \sigma$ for some $\alpha\ge 0$}
\\
&=
m\(d^{\nicefrac{1}{2}}\exp{\beta \alpha_2\[\frac{d\beta^2}{2}\]^{\nicefrac{1}{2}}}
-1
\)
\end{align}
\end{claim}


\begin{align}
\norm{\calT_{\text{Dense}}\(\bx\)-\bxi_\mu}&\ge 
m\(d^{\nicefrac{1}{2}}\exp{\beta \Max_{\mu\in [M]}\Braket{\bxi_\mu,\bx}-\beta^2d}
-1
\)\\
&=
m\(d^{\nicefrac{1}{2}}\exp{\beta \alpha_2\sigma}
-1
\), \quad\text{for some } \alpha_2\ge 0\\
&=
m\(d^{\nicefrac{1}{2}}\exp{\beta \alpha_2\(\frac{d\beta^2}{2}\)^{\nicefrac{1}{2}}}
-1
\)
\\
\norm{\calT\(\bx\)-\bxi_\mu}&\le
m\(1+\beta \[\beta d+\alpha_1\(\frac{d\beta^2}{2}\)^{\nicefrac{1}{2}}\]\)
\le 
m\(1+ \beta \abs{\Max_{\mu\in [M]}\Braket{\bxi_\mu,\bx}}\)
\end{align}
}


\begin{theorem}
In the low temperature region, $\beta\to \infty$, the number of patterns randomly sampled from a
sphere of radius $m$ that the sparse Hopfield model can store and retrieve is lower-bounded by
\bea
M_{Max} \ge 2\sqrt{\pi}\frac{(\beta-1)m^2+2Rm+1-\frac{R}{m}}{m^2 \sqrt{\frac{2}{d}}}\exp\Bigg\{\frac{\[(\beta-1)m^2+2Rm+1-\frac{R}{m}\]^2}{m^4 \frac{2}{d}}\Bigg\}
\eea
\end{theorem}
\begin{proof}
\mattcomment{Directly compute based on the strong assumption setting given by Jerry}
With theorem \cref{thm:well_separation}, we write down the probability of success storage and retrieval
\bea
P\(\Delta_{\mu\nu} \ge 1+\beta m^2+2mR-\frac{R}{m}\) \\
=P\(m^2-\Theta_{\mu\nu} \ge 1+\beta m^2+2mR-\frac{R}{m}\) \\
=P\(\Theta_{\mu\nu} \le (1-\beta)m^2-2Rm-1+\frac{R}{m}\)
\eea
Applying the distribution $\Theta \sim N(0,\nicefrac{m^4}{d})$, we obtain
\bea
P\(\Theta_{\mu\nu} \le (1-\beta)m^2-2Rm-1+\frac{R}{m}\) \\
=\half\(1+\mathsf{erf}\(\frac{(1-\beta)m^2-2Rm-1+\frac{R}{m}}{m^2 \sqrt{\frac{2}{d}}}\)\)\\
=\half\(1-\mathsf{erf}\(\frac{(\beta-1)m^2+2Rm+1-\frac{R}{m}}{m^2 \sqrt{\frac{2}{d}}}\)\)\\
=\half\mathsf{erfc}\(\frac{(\beta-1)m^2+2Rm+1-\frac{R}{m}}{m^2 \sqrt{\frac{2}{d}}}\)
\eea
The probability of having a pair to satisfy \cref{def:stored_and_retrieved} is thus
\bea
P\(\Delta_{\mu\nu} \ge 1+\beta m^2+2mR-\frac{R}{m}\)=\half\mathsf{erfc}\(\frac{(\beta-1)m^2+2Rm+1-\frac{R}{m}}{m^2 \sqrt{\frac{2}{d}}}\).
\eea
The average number of samples of $\Delta_{\mu\nu}$ one needs to draw before a sample satisfies \cref{def:stored_and_retrieved} is given by
\bea
P\(\Delta_{\mu\nu} \ge 1+\beta m^2+2mR-\frac{R}{m}\)^{-1},
\eea
and the expected maximum number of patterns that the model can store is hence
\bea
\label{eqn:M_Max}
M_{Max}=2\mathsf{erfc}\(\frac{(\beta-1)m^2+2Rm+1-\frac{R}{m}}{m^2 \sqrt{\frac{2}{d}}}\)^{-1}.
\eea
Then we want to estimate the value of $\mathsf{erfc}$ function. For sufficient large $x$, the $\mathsf{erfc}$ function can be accurately approximated by asymptotic expansion
\bea
\mathsf{erfc}(x) \approx \frac{e^{-x^2}}{\sqrt{\pi}x}\sum^\infty_{i=0} (-1)^n\frac{(2i-1)!!}{\(2x^2\)^n}.
\eea
While $M$ is sufficient large, with the inverse zero-order expansion we can obtain a tight lower bound of $\mathsf{erfc}^{-1}$:
\bea
\label{eqn:erfc_bound}
\mathsf{erfc}(x)^{-1} \ge \sqrt{\pi}xe^{x^2}.
\eea
We utilize the lower bound in \eqref{eqn:erfc_bound} in \eqref{eqn:M_Max} to obtain the average maximum number of patterns that the model can store
\bea
M_{Max} \ge 2\sqrt{\pi}\frac{(\beta-1)m^2+2Rm+1-\frac{R}{m}}{m^2 \sqrt{\frac{2}{d}}}\exp\Bigg\{\frac{\[(\beta-1)m^2+2Rm+1-\frac{R}{m}\]^2}{m^4 \frac{2}{d}}\Bigg\}
\eea
\end{proof}
{\color{black!50}
To compute the \textit{tightest} upper bound of $\norm{\calT(\bx)-\bxi}$, we need the \textit{largest} $\kappa(\bz)$ (the rank of smallest non-zero output of $\Sparsemax(\bz)$), which is defined as
\bea
\kappa(\bz) = \Max \bigg\{ k\in[M]\;\bigg\vert\; 1+kz_{(k)}>\sum_{\nu\le k} z_{(\nu)} \bigg\},
\eea
with $z_{(\nu)}$ the $\nu$'th element in a sorted descending $z$-sequence $\bz_{\text{sorted}}\coloneqq z_{(1)}\ge z_{(2)}\ge\ldots\ge z_{(M)}$ and 
$$z  \sim N\(\beta d,\frac{d\beta^2m^2}{2}\).$$
}
\end{proof}








\subsection{High Assumption Results: low temperature region with assumptions on pattern distribution}
Here we provide more detailed characterization of $M$ by imposing strong assumptions.
Formally, \cref{coro:convergence_sparse} ensures error-free retrieval in the low-temperature region, as $\beta \to \infty$, provided that the well-separation condition is met. This is because $\beta$ governs the steepness of the energy landscape surrounding the target memory pattern.
\begin{theorem}
In the low temperature region, $\beta\to \infty$, the number of patterns randomly sampled from a
sphere of radius $m$ that the sparse Hopfield model can store and retrieve is lower-bounded by
\bea
M_{Max}\ge 2\sqrt{\pi}\frac{m^2-\frac{1}{\beta}\ln(\frac{2(M-1)m}{R})-2mR}{m^2\sqrt{\frac{2}{d}}} \exp\Bigg\{\frac{\[m^2-\frac{1}{\beta}\ln(\frac{2(M-1)m}{R})-2mR\]^2}{m^4\frac{2}{d}}\Bigg\}
\eea
\end{theorem}
\begin{proof}
\normalsize
Let $\theta_{\mu\nu}$ be the angle between two patterns $\bxi^\mu,\bxi^\nu\in\R^d$.
Intuitively, $\theta_{\mu\nu}\in[0,\pi]$ represent the pairwise correlation of two patterns the two patterns.
Let $\phi_{\mu\nu}\coloneqq\norm{\bxi_\mu-\bxi_\nu}$ be the Euclidean distance between $\bxi_\mu,\bxi_\nu$.
Observe
\bea
\norm{\bxi_\mu-\bxi_\nu}=\[2m -2\Braket{\bxi_\mu,\bxi_\nu}\]^\half
\leq \[2m -2m^2 \cos{\theta_{\mu\nu}}\]^\half
,
\eea
and moreover, for $\bxi_\mu,\bxi_\nu$ sampled from the same spherical distribution, $\{\rho_{\mu\nu}\coloneqq\Braket{\bxi_\mu,\bxi_\nu}/m^2\}$ are pairwise i.i.d. according to \cite[Lemma~4.1]{cai2012phase}
\bea
P(\rho)=\frac{\Gamma\(\frac{d}{2}\)}{\sqrt{\pi}\Gamma\(\frac{d-1}{2}\)}\(1-\rho^2\)^{\frac{d-3}{2}}.
\eea
Notably, while $\{\rho_{\mu\nu}\}$ are pairwise iid, the patterns in the same pair are mutually dependent. 
\red{However, as pointed out in \cite{cai2012phase}, 
for large $d$ and $M$, the dependence between patterns can be ignored.}
By taking the large $d$ limit, we have
\bea
P(\rho)\to \frac{1}{\sqrt{2\pi}(\sqrt{\nicefrac{1}{d}})}\exp{-\half\(\frac{\rho}{\sqrt{\nicefrac{1}{d}}}\)^2},
\eea
where the identity $\lim_{d\to \infty} {\Gamma\(\frac{d}{2}\)}/{\Gamma\(\frac{d-1}{2}\)} \simeq \sqrt{\nicefrac{d}{2}}$ is used.
Let $\Theta\coloneqq m^2\rho$ be the random variable representing the inner product $\{\Braket{\bxi_\mu,\bxi_\nu}\}$, we have
\bea
P(\Theta)=\frac{1}{\sqrt{2\pi}(m^2 \sqrt{\nicefrac{1}{d}})}\exp{-\half\(\frac{\rho}{m^2\sqrt{\nicefrac{1}{d}}}\)^2},\quad 
\eea
where implies 
\bea
\phi= \sqrt{2m-2\Theta} \sim N\(\sqrt{2m}, \frac{2m^2}{\sqrt{d}}\) \text{and } \Theta\sim N(0,m^4/d).
\eea
Let 
$
\Delta_{\mu\nu}= \Braket{\bxi_\mu,\bxi_\mu} -  \Braket{\bxi_\mu,\bxi_\nu}
$.
Note that, $\Delta_{\mu\nu}\ge \Delta_{\mu}$.
Therefore, we can generalize the well-separation condition to
\bea
\Delta_{\mu\nu}\ge \Delta_{\mu} \ge \frac{1}{\beta}\ln\(\frac{2(M-1)m}{R}\)+2mR,
\eea
where 
\bea
\Delta_{\mu\nu} = m^2-\Theta_{\mu\nu}.
\eea

Let $\bX\sim N(\mu, \sigma)$ and \red{$L<\mu$}.
{\color{black!50}
The CDF of $x\sim N(\mu,\sigma^2)$:
\bea
\Phi\(x\)=\frac{1}{\sqrt{2\pi}}\int_{-\infty}^x \dd t\; \exp{-\half t^2}.
\eea
and
\bea
\Phi\(\frac{x-\mu}{\sigma}\)=\frac{1}{\sqrt{2\pi}}\int_{-\infty}^x \dd t\; \exp{-\half \(\frac{t-\mu}{\sigma}\)^2}.
\eea
The error function:
\bea
\mathsf{erf}\(x\)\coloneqq \frac{2}{\sqrt{\pi}}\int_0^x \dd t\; e^{-\half t^2},
\eea
and 
\bea
\mathsf{erfc}(x)\coloneqq 1- \mathsf{erf}\(x\).
\eea
Note that $\mathsf{erf}(-x)=-\mathsf{erf}(x)$.

Therefore,
\bea
\Phi(x)=\half\[1+\mathsf{erf}\(\frac{x}{\sqrt{2}}\)\].
\eea

\bea
P\(X\le L\)&=&\half +\half \mathsf{erf}\(\frac{L-\mu}{\sqrt{2}\sigma}\)
=\half \[1-\mathsf{erf}\(-\frac{L-\mu}{\sqrt{2}\sigma}\)\]\\
&=&
\half \[1-\mathsf{erf}\(\frac{\mu-L}{\sqrt{2}\sigma}\)\]
=
\half\mathsf{erfc}\(\frac{\mu-L}{\sqrt{2}\sigma}\).
\eea


Therefore, at large $d$ limit, the probability for the randomly sampled pattern pair to be well-stored is
\begin{align}
P\(\phi \le 2R \)&= \frac{1}{\sqrt{2\pi}\(\sqrt{2}md^{-\nicefrac{1}{4}}\)}\int_0^{2R}\dd t \; \exp{-\half\(\frac{\sqrt{2m}t-\sqrt{2m}}{\sqrt{2}md^{-\nicefrac{1}{4}}}\)^2}\\
&=
\end{align}
}

{\color{firebrick}

We want to see that, under the large $d$ limit, the \textit{expected} number of patterns $M$ can be well-stored and retrieved  into the model before a sampled pattern pair violates the storage definition \cref{def:stored_and_retrieved}. Intuitively, the inverse failure probability is the expected maximum numbers of well-stored patterns.

Given $\Theta\sim N(0,m^4/d)$, the probability of having a pair to violate \cref{def:stored_and_retrieved} is
\begin{itemize}
    \item Weak (just storage, the same as Kernel memory paper without touching sparse Hopfield model):
    \bea
    P\(\phi\le 2R\)
    \eea
    \item Failure Probability (storage and retrieval):
    \begin{align}
    \label{eqn:violation_prob}
    &P\(m^2-\Theta_{\mu\nu} = \Delta_{\mu\nu}\le \Delta_{\mu} \le \frac{1}{\beta}\ln\(\frac{2(M-1)m}{R}\)+2mR\)\\
    &=P\(m^2-\Theta_{\mu\nu} \leq \frac{1}{\beta}\ln(\frac{2(M-1)m}{R})+2mR\)\\
    &=P\(\Theta_{\mu\nu}\geq m^2-\frac{1}{\beta}\ln(\frac{2(M-1)m}{R})-2mR\)  
    \end{align}
\end{itemize}
Applying the distribution $\Theta \sim N(0,\nicefrac{m^4}{d})$, we have
\bea
&P&\(\Theta_{\mu\nu} \ge m^2-\frac{1}{\beta}\ln(\frac{2(M-1)m}{R})-2mR\)\\
&=&\half\Bigg\{1-\mathsf{erf}\[\frac{m^2-\frac{1}{\beta}\ln(\frac{2(M-1)m}{R})-2mR}{m^2\sqrt{\frac{2}{d}}}\]\Bigg\}\\
&=&\half \mathsf{erfc}\Bigg\{\frac{m^2-\frac{1}{\beta}\ln(\frac{2(M-1)m}{R})-2mR}{m^2\sqrt{\frac{2}{d}}}\Bigg\}
\eea
The probability of having a pair to violate \cref{def:stored_and_retrieved} is thus
\bea
P \(\Delta_{\mu\nu}\leq \frac{1}{\beta}\ln(\frac{2(M-1)m}{R})+2mR\)=\half \mathsf{erfc}\Bigg\{\frac{m^2-\frac{1}{\beta}\ln(\frac{2(M-1)m}{R})-2mR}{m^2\sqrt{\frac{2}{d}}}\Bigg\}
\eea
\bea
\Delta_\mu = \Min_\nu \Braket{\bxi_\mu, \(\bxi_\mu-\bxi_\nu\) }
\eea
The average number of samples of $\Delta_{\mu\nu}$ one needs to draw before a sample satisfies \cref{def:stored_and_retrieved} is given by
\bea
P \(\Delta_{\mu\nu}\le \frac{1}{\beta}\ln(\frac{2(M-1)m}{R})+2mR\)^{-1},
\eea
and the expected maximum number of patterns that the model can store is hence
\bea
\label{eqn:Expected M Max}
M_{Max}=2\mathsf{erfc}\Bigg\{\frac{m^2-\frac{1}{\beta}\ln(\frac{2(M-1)m}{R})-2mR}{m^2\sqrt{\frac{2}{d}}}\Bigg\}^{-1}.
\eea
Then we want to estimate the value of $\mathsf{erfc}$ function. For sufficient large $x$, the $\mathsf{erfc}$ function can be accurately approximated by asymptotic expansion
\bea
\mathsf{erfc}(x) \approx \frac{e^{-x^2}}{\sqrt{\pi}x}\sum^\infty_{n=0} (-1)^n\frac{(2n-1)!!}{\(2x^2\)^n}.
\eea
While $d$ is sufficient large, with the inverse zero-order expansion we can obtain a tight lower bound of $\mathsf{erfc}^{-1}$:
\bea
\label{eqn:inverse erfc lower bound}
\mathsf{erfc}(x)^{-1} \ge \sqrt{\pi}xe^{x^2}.
\eea
We utilize the lower bound in \eqref{eqn:inverse erfc lower bound} in \eqref{eqn:Expected M Max} to obtain the average maximum number of patterns that the model can store
\bea
M_{Max}\ge 2\sqrt{\pi}\frac{m^2-\frac{1}{\beta}\ln(\frac{2(M-1)m}{R})-2mR}{m^2\sqrt{\frac{2}{d}}} \exp\Bigg\{\frac{\[m^2-\frac{1}{\beta}\ln(\frac{2(M-1)m}{R})-2mR\]^2}{m^4\frac{2}{d}}\Bigg\}.
\eea

\jhcomment{We tried but turned out to be wrong. $M_{\Max}$ should not depend on $M$, sadly.}
\begin{claim}
    \textbf{TODO:} Knowing $\Theta\sim N(0,m^4/d)$ under large $d$ limit, use \eqref{eqn:violation_prob} (especially the properties of error function) to derive the \textit{expected} maximum number of patterns satisfying the well-separation condition.
\end{claim}
\textbf{Possible Solutions:}
\begin{enumerate}
    \item Properties of Error Function.
    \item Exponential Chebyshev's inequality:
    \bea
    P\(X\ge \epsilon\)\le e^{-t\epsilon}\E\[\exp{tX}\],\quad t>0.
    \eea
\end{enumerate}
}

\paragraph{Method 2: Exponential Chebyshev's inequality.}

    By $\Theta\sim N(0,m^4/d)$, we have
    \begin{align}
    \E\[\exp{t\Theta}\]=\exp{\half \frac{m^4}{d}t^2},
    \end{align}
    where exponential normal identity $\E\[\exp{tZ}\]=\exp{\mu t +\sigma^2t^2/2}$ with $Z\sim N(\mu,\sigma^2)$ is used.
    Therefore,
    \begin{align}
    P&\(\Theta\geq m^2-\frac{1}{\beta}\ln(\frac{2(M-1)m}{R})-2mR\)\\
    &\le \exp{-t \[m(m-2R) -\frac{1}{\beta}\ln(\frac{2(M-1)m}{R})\]} \exp{\half \frac{m^4}{d}t^2},     
    \end{align}

    





\end{proof}
